Skill-Critic: Refining Learned Skills for Hierarchical Reinforcement Learning

Hierarchical reinforcement learning (RL) can accelerate long-horizon decision-making by temporally abstracting a policy into multiple levels. Promising results in sparse reward environments have been seen with skills, i.e. sequences of primitive actions. Typically, a skill latent space and policy are discovered from offline data. However, the resulting low-level policy can be unreliable due to low-coverage demonstrations or distribution shifts. As a solution, we propose the Skill-Critic algorithm to fine-tune the low-level policy in conjunction with high-level skill selection. Our Skill-Critic algorithm optimizes both the low-level and high-level policies; these policies are initialized and regularized by the latent space learned from offline demonstrations to guide the parallel policy optimization. We validate Skill-Critic in multiple sparse-reward RL environments, including a new sparse-reward autonomous racing task in Gran Turismo Sport. The experiments show that Skill-Critic's low-level policy fine-tuning and demonstration-guided regularization are essential for good performance. Code and videos are available at our website: https://sites.google.com/view/skill-critic.

==> sections/experiments_archive.tex <==

% =============== experiments ===========
\section{Experiments} \label{Sec:Exp}
Our experiments aim to answer: (1) Can Skill-Critic effectively leverage low-coverage, low-quality demonstrations to accelerate downstream RL? (2) Is the proposed LL policy update step necessary in improving the skill set and optimizing the agent performance in the downstream task?  

% ===================== env intro ================
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.76942\textwidth]{figures/EnvFigs2.pdf}
    \caption{For each environment, we collect an offline dataset for skill training (\textbf{left}), and test skill improvement on more complex target tasks (\textbf{right}). The agent must use short navigation skills to guide it through a diagonal maze or complicated trajectory planning (\textbf{top}), and use low-velocity trajectories to navigate a corner of the racetrack as quickly as possible (\textbf{bottom}).}
    \label{fig:EnvFigs}
\end{figure*}

\begin{figure}[t]
    \centering
    \subfigure[Table Cleanup]{
    \includegraphics[width=.45\columnwidth]{figures/slipperpush.png}}
        \subfigure[Slippery Push]{
    \includegraphics[width=.45\columnwidth]{figures/slipperpush.png}}
    \caption{\textbf{\color{black}{Robotic Arm Evaluation Environment}}\color{black}{ proposed by Rana et al \cite{rana2023residual}. A MuJoCO-based \cite{todorov2012mujoco} 7-DoF Fetch robotic arm interacts with objects placed in front of it to place a block on a tray in the scene (Table Cleanup) or push a block along a slippery table to a goal (Slippery Push).}}
    \label{fig:fetcharm}
\end{figure}

\subsection{Environments, Tasks, and Demonstrations} \label{Subsec: Exp env} We evaluate Skill-Critic in three tasks: maze navigation, maze trajectory planning, and autonomous racing (Fig.~\ref{fig:EnvFigs}). We collect a large dataset of demonstrations that can create an informative skill set; however, the skill set does not contain \textit{all} of the potential skills that may aid downstream tasks. We evaluate the environment reward, to test not only whether the task is completed, but also how well the task is completed.
% instead of a simple task success rate. 

% Appendix~\ref{Appendix: env} contains a full description of environments and data collection.

{\bf Maze Navigation.}
The maze navigation task is based on the D4RL point maze environment~\cite{fu2020d4rl} that uses a top-down agent-centric state and 2D velocity as the action. We use the same planner-based demonstrations as~\cite{pertsch2021accelerating}, consisting of 85000 goal-reaching trajectories in randomly generated, small maze layouts. We create a new maze navigation task with multiple diagonal tunnels (see Fig.~\ref{fig:EnvFigs}) for downstream learning. The agent has 2000 steps in each episode and receives a binary reward for each time-step that the distance to the goal is below a threshold, encouraging the agent to reach the goal in fewer steps. The agent can transfer skills such as traversing hallways or passing through doors.
% , but must learn to rapidly navigate the diagonal maze. 
% The state consists of an RGB top-down view centered around the agent augmented with the time since the last skill was completed, $k$.


{\bf Maze Trajectory Planning.}
The maze trajectory planning task uses the same skills, simulation engine, episode length, and reward as the maze navigation task. The difference is that the downstream environment has a curvy tunnel with corners of varying shapes, offering the agent multiple options for position, heading, and velocity.  To minimize time to reach the goal, the agent must learn to create 
a smooth trajectory specialized to the full course.

\begin{newtext}
\textbf{Robot Manipulation: } We implement robot manipulation experiments on a 7-DoF Fetch robotic arm simulated in MuJoCO \cite{todorov2012mujoco}. We directly use two tasks proposed in Rana et al. \cite{rana2023residual} as shown in Fig. \ref{fig:fetcharm}. We use the demonstration data consisting of 40k trajectories provided by Rana et al. \cite{rana2023residual}, which was collected with handcrafted controllers. 
For \emph{Slippery Push} task, the agent is required to push a block to a given goal, but the friction of the table surface is lowered from that seen in the demonstrations. The agent receives a reward of 1 once the block is at the goal location, otherwise the reward is 0. The task is episodic and terminates after 100 steps. 
For \emph{Table Cleanup} task, the agent must place a block on a rigid tray object, which was not present in the demonstrations. The agent receives a reward of 1 only when the block is placed on the tray, otherwise the reward is 0. The task is episodic and terminates after 50 steps.
\end{newtext}

{\bf Autonomous Racing.}
We employ the Gran Turismo Sport (GTS) high-fidelity racing simulator~\cite{fuchs2021super} to test a new, sparse reward autonomous racing task. The low-dimensional state representation includes pose, velocity, and track information. There are two continuous actions: steering angle and a combined throttle/brake command between $[-1,1]$. Unlike previous works in GTS~\cite{fuchs2021super, wurman2022outracing}, we create a sparse reward to navigate a single corner. The agent starts at a low speed in the center of the track and has 600-step (60-sec) episodes; the agent receives a binary +1 reward for every time step when it passes the finish line.  For demonstrations, we use GTS's built-in AI controller to collect 40000 trajectories from random, low-speed starting points on the course, each 200 steps in length. While the built-in AI is capable of controlling the race car at high-speed, we deliberately bias the demonstration toward low-speed maneuvers to test Skill-Critic's ability to improve skills. The agent can transfer skills such as speeding up and turning from the low-speed demonstrations but must improve these skills to complete the corner as fast as possible.
% In the downstream RL task, suboptimal skills hinder fast and collision-free trajectory planning. These demonstrations navigate the corner, but are suboptimally slow.

{\bf Baselines.} We compare Skill-Critic with existing methods to show the necessity of fine-tuning a temporally abstracted LL policy. \textbf{SAC} performs model-free RL via SAC~\cite{haarnoja2018soft} without offline experience or temporal abstraction. \textbf{BC+SAC} uses offline experience to initialize a policy with behavioral cloning (BC), then fine-tune the policy via SAC. \textbf{SPiRL}~\cite{pertsch2021accelerating} extracts temporally extended skills with a skill prior from the offline data, but downstream RL training occurs only on the HL skill selection policy. Our version of SPiRL uses a state-dependent policy to improve performance~\cite{pertsch2021guided}. 
\begin{newtext}
\textbf{ReSkill}~\cite{rana2023residual} is a hierarchical RL method that uses residual skill policies to augment the stationary LL policy during training rather than directly fine-tuning the learned LL policy.
\end{newtext}

% =============== main results ==============




\subsection{Experimental Results} \label{Subsec: ExpMazeNav}

{\bf Maze Navigation and Trajectory Planning.} 
We analyze the maze tasks in Figure~\ref{fig:MazeResults}. In both tasks, SAC and BC+SAC fail to reach the goal, likely since the single-step policy is unable to discover the sparse reward. In comparison, the temporally abstracted methods (SPiRL and Skill-Critic) can effectively utilize offline demonstrations to successfully find and reach the goal. However, SPiRL plans slow, jagged trajectories because it cannot improve the offline-learned skills. We warm-start Skill-Critic with SPiRL after 1M steps to stabilize the HL policy, and Skill-Critic is then able to further optimize its path, resulting in planning an optimal trajectory. Skill-Critic \textit{discovers} diagonal motion, but it does not forget the skills to solve the maze due to the LL policy regularization. This regularization is crucial to  guide exploration.
% (ablations in Appendix~\ref{Appendix: Ablation}).

\begin{figure*}[t]
    \centering
        \includegraphics[width=0.4\textwidth]{figures/maze.pdf}
    \includegraphics[width=0.4\textwidth,trim={25cm 0 0 0},clip]{figures/MazeExp.pdf}
    \caption{Maze experiment results. \textbf{Left:} average episode rewards with 3 random seeds. Skill-Critic begins training at 1 million steps and is warm-started by SPiRL. \textbf{Right:} SPiRL and Skill-Critic trajectories at convergence. SPiRL reuses right-angle movements from the skills, resulting in slow, jagged paths. Skill critic discovers new skills to plan diagonal trajectories.}
    \label{fig:MazeResults}
\end{figure*}

\begin{newtext}
{\bf Robot Manipulation}. We provide the results for the 7-DoF Fetch arm tasks in Fig. \ref{fig:fetchresults}. As originally shown in the original paper \cite{rana2023residual}, ReSkill quickly learns a policy to clean the table, and outperforms other hierarchical methods like Hierarchical Actor Critic (HAC) \cite{levy2018learning} and PARROT \cite{singh2020parrot}, which are unable to learn anything meaningful on the task (see results in \cite{rana2023residual}). The alternative skill-embedding space in ReSkill speeds up exploration by biasing the HL policy towards skills relevant to the state. However, the LL residual policy in ReSkill only improves its value through the single-step reward $r(s,a)$. Skill-Critic can achieve an even higher reward by completing the task even \textit{faster}. We attribute this to the inter-related Q-function update that estimates the LL Q-function using the $H$-step reward estimate \textit{upon arrival} to a skill (refer to \ref{Eqn: Qatau} and \ref{Eqn: Qat} in the text). Thus, the sparse reward is able to propagate further into the LL policy update, resulting in higher rewards. An interesting area for future research would be to apply ReSkill's alternative skill embedding to Skill-Critic to accelerate training.  However, we believe Skill-Critic's LL policy update is crucial to converge to the highest reward.
\end{newtext}

\begin{figure}[t]
    \centering
        \subfigure[Table Cleanup]{
    \includegraphics[width=.46\columnwidth]{figures/cleantable.pdf}}
            \subfigure[Slippery Push]{
    \includegraphics[width=.46\columnwidth]{figures/slippery_rew.pdf}}
    \caption{\textbf{\color{black}{Evaluation on 7DoF Robotic Arm. }} \color{black}{Mean episode reward (std) for each environment. Skill-Critic is warm-started with SPiRL at 500k steps.  Note how Skill-Critic achieves a higher reward.}}
    \label{fig:fetchresults}
\end{figure}

{\bf Autonomous Racing}. \label{Subsec: ExpRacing}
In Fig.~\ref{fig:RaceResults}, we evaluate the performance of RL training in the autonomous racing task using the episode reward and time in contact with the wall on the edge of the track. Further, we analyze the trajectories from each method's highest reward policy. 
SAC sufficiently explores to eventually reach the goal, but is slow to improve its policy with the sparse reward, resulting in policies with relatively low velocity. Warm-starting the SAC policy appears to hinder exploration; in fact, BC+SAC is unable to find the goal, and its trajectories consistently crash within the first straight-away.
In contrast, SPiRL makes use of the pre-trained skills, allowing it to exploit skills that can consistently reach the goal. However, these skills are learned from low-speed demonstrations. Thus, SPiRL's HL policy cannot generate high-speed trajectories given the stationary LL policy that is only capable of low-speed maneuvers. Plus, since the demonstration is limited in diversity, the offline learned skills suffer from distributional shifts. As a result, SPiRL frequently collides with the wall throughout the corner. All these factors prevent SPiRL from further improving its performance.

\begin{figure*}[t]
    \centering
    \includegraphics[width=.85\textwidth]{figures/gts_without_hitting_velocity.pdf}
    \caption{Autonomous racing results in Gran Turismo Sport. \textbf{Top left:} mean (std) episode reward. \textbf{Bottom left:} mean (std) of cumulative time in contact with wall at track boundary per episode (bottom). \textbf{Right:} Visualization of the trajectories from each method's highest scoring policy. Car markers indicate location at various times. Inset plot shows velocity vs. position along the track.}
    \label{fig:RaceResults}
\end{figure*}

Skill-Critic addresses these issues with online LL policy training, achieving higher episode rewards, reducing contact time with course walls, and quickly navigating the corner. Skill-Critic exploits the offline pre-training and temporally extended actions to guide exploration. Furthermore, the LL fine-tuning allows the Skill-Critic agent to navigate at a high velocity, which requires complex maneuvers like avoiding collision and slowing and turning hard in the corner. For reference, we compare the performance to GTS's Built-in AI, which is a high-quality, rule-based controller deployed with the game as a competitor for players. Note that Skill-Critic only has access to low-speed demonstrations from Built-in AI, and we use a \emph{sparse} reward, unlike previous methods with hand-engineered dense rewards~\cite{wurman2022outracing}. Given these factors, we consider Built-in AI a strong baseline for this single-corner racing task. Despite this, the Skill-Critic policy can consistently perform as well as the Built-in AI.

\begin{newtext}
    
\subsection{Ablation Study} \label{subsec: ablation}

\begin{figure}[t]
    \centering
   {\sffamily Target Divergence (td)}\\
    \includegraphics[width=.46\columnwidth,trim={0 0 24.5cm 1cm},clip]{figures/Ablation.pdf} \includegraphics[width=.46\columnwidth]{figures/maze2_KD.pdf}
    \caption{Ablation study of LL policy regularization in the Maze Navigation task. All agents are warm-started by SPiRL for 1 million steps. \textbf{Left:} LL policy target KL divergence, $\delta_a$. \textbf{\color{black}{Right:}} \color{black}{LL policy's actual KL divergence from the action prior during training.}}
    \label{fig:Ablation_kl}
\end{figure}

\begin{figure}[t]
    \centering
        \includegraphics[width=0.92\columnwidth,trim={12.5cm 0 0 0},clip]{figures/Ablation.pdf}
    \caption{Ablation study of LL action prior variance in the Maze Navigation task. All agents are warm-started by SPiRL for 1 million steps. \textbf{Left:} Prior distribution for LL policy regularization: uniform prior (entropy) or proposed non-uniform prior (KL divergence).  \textbf{Right:} LL policy initial variance, $\sigma_{\hat{a}}$. }
    \label{fig:Ablation}
\end{figure}

In this section, we examine the effect of the regularization for the LL policy and its effect on the overall performance of the skill critic algorithm. As we have described in Section \ref{Sec:HRLregularize}, the LL policy is regularized by the action prior, which is informed by the pre-trained decoder. 
In the experiments in Fig. \ref{fig:Ablation_kl} and Fig. \ref{fig:Ablation}, we demonstrate that it is necessary to regularize the LL policy with the action prior using KL divergence, and analyze the effect of related hyperparameters. 

\textbf{LL Target KL Divergence.} In Fig. \ref{fig:Ablation_kl}, we compare varying values for the low-level policy target KL divergence, $\delta_a$.
% as described in Appendix \ref{Appendix: downstream RL}. 
The target divergence $\delta_a$ is used to determine the parameter, $\alpha_a$, which determines the effect of the KL regularization term in the policy update objective as described in \cite{haarnoja2018soft, pertsch2021accelerating}. We compare $\delta_a$ values 10, 20, 50 and 80 for the maze navigation experiment corresponding to Fig. \ref{fig:MazeResults}. All methods are warm-started with SPiRL for 1M steps. Then they are trained via Skill-Critic with the varying value for $\delta_a$. The results show that when target divergence increases, the episode rewards increase correspondingly, because the LL policy has more freedom to deviate from the prior policy. Conversely, a smaller target divergence constrains the policy closer to the action prior, and Skill-Critic receives less reward. Furthermore, we provide the actual KL divergence of the LL policy from the action prior during training in the right of Fig. \ref{fig:Ablation_kl}. As explained on Line 9 in Algorithm \ref{Alg:low-level}, $\alpha_a$ is the dual gradient descent parameter to constrain the LL policy's divergence to the target divergence $\delta_a$. From the actual LL policy variance during training, we can see that the LL policy divergence is indeed constrained to the target divergence and converges to the target divergence value.

\textbf{LL Prior Distribution.} Skill-Prior RL \cite{pertsch2021accelerating} extends the uniform prior in SAC~\cite{haarnoja2018soft} to the non-uniform HL skill prior. Skill-Critic likewise employs a non-uniform action prior learned from demonstration to regularize the LL policy exploration. We conduct an ablation study in the maze navigation task using a uniform LL prior, which replaces the KL divergence regularization term with LL policy entropy. The results of the learning curves are provided in Fig. \ref{fig:Ablation}. We apply the auto entropy adjustment and use the target entropy value of -2~\cite{haarnoja2018soft2}. However, the uniform prior regularizes the LL policy to execute random actions, leading to inefficient exploration in the long-horizon environment.

\textbf{Variance of the Action Prior.} In Fig. \ref{fig:Ablation}, we change the variance of the action prior, $\sigma_{\hat{a}}$ to values $\log \sigma_{\hat{a}}=-1$, $-3$, and $-5$ in the maze navigation task. All methods are warm-started with SPiRL for 1M steps. Then they are trained via Skill-Critic with the varying value for $\sigma_{\hat{a}}$. When the variance is too small ($\log \sigma_{\hat{a}}=-5$), the LL policy is unable to sufficiently explore to improve its skills. Conversely, larger variance, i.e. $\log \sigma_{\hat{a}}=-1$, means the low-level policy explores with weaker regularization to the action prior, so the agent forgets previous skills and fails to reach the goal. We found a suitable value for the action-prior variance is $\log \sigma_{\hat{a}}=-3$, which promotes reasonable exploitation of the action prior and policy exploration to improve the skill set.

\end{newtext}



==> submit1/submittedRAL/abstract.tex <==
\begin{abstract}
Hierarchical reinforcement learning (RL) can accelerate long-horizon decision-making by temporally abstracting a policy into multiple levels. 
Promising results in sparse reward environments have been seen with \textit{skills}, i.e. sequences of primitive actions. Typically, a skill latent space and policy are discovered from offline data. However, the resulting low-level policy can be unreliable due to low-coverage demonstrations or distribution shifts.
As a solution, we propose the \emph{Skill-Critic} algorithm to fine-tune the low-level policy in conjunction with high-level skill selection. Our Skill-Critic algorithm optimizes both the low-level and high-level policies; these policies are initialized and regularized by the latent space learned from offline demonstrations to guide the parallel policy optimization. We validate our approach in multiple sparse RL environments, including a new sparse reward autonomous racing task in Gran Turismo Sport. The experiments show that Skill-Critic's low-level policy fine-tuning and demonstration-guided regularization are essential for good performance. Code and videos are available at \href{https://sites.google.com/view/skill-critic}{https://sites.google.com/view/skill-critic}. 
\end{abstract}

% \begin{IEEEkeywords}
% Hierarchical Reinforcement Learning, Skill Learning, Transfer Learning
% \end{IEEEkeywords}

==> submit1/submittedRAL/approach.tex <==


% =============== approach ==============
\section{Approach} \label{Sec:Approach}
Our goal is to employ demonstration-informed, temporally abstracted skills in hierarchical RL to facilitate the learning of complex long-horizon tasks~\cite{pertsch2021accelerating}. Ultimately, we aim to solve the task with a hierarchical policy, consisting of 1) a high-level (HL) policy, $\pi_z(z_t|s_t)$, that selects the best skill, $z_t$, given the current state, $s_t$; and 2) a low-level (LL) policy, $\pi_a(a_t|s_t,z_t)$, selects the optimal action, $a_t$, based on the current state and selected skill. The HL policy selects skills from a learned continuous skill set $\mathcal{Z}$, i.e., $z_t\in\mathcal{Z}$. As in SPiRL~\cite{pertsch2021accelerating}, we consider the setting in which we can extract an initial skill set from offline demonstrations to accelerate downstream RL training. We further consider the case when the extracted skill set is \emph{insufficient} for solving the downstream tasks, which motivates our \textit{Skill-Critic} framework. The proposed framework is detailed in Figure~\ref{fig:framework}, which consists of two stages. In Stage 1, we leverage demonstrations to learn a skill decoder and skill prior that can accelerate RL training. In Stage 2, we leverage hierarchical RL to fine-tune \emph{both} the HL and LL policies, thus, further improving the inadequate offline learned skill set.



%comment
\subsection{Offline Skill Prior and Embedding Pre-Training (Stage 1)}\label{Sec:skillprior}
We assume access to demonstrations in the training environment consisting of trajectories $\mathcal{D}=(\tau_0, \tau_1, ..., \tau_N)$, which each include states and actions at every time step $\tau=(s_t, a_t, ...)$. The demonstrations may not contain complete solutions for the downstream task; this motivates transferring skills by training an HL policy to select the best skills for a new task. We furthermore consider the case when demonstrations include only a subset of potential skills or suboptimal skills,  motivating the improvement of skills with RL fine-tuning of the LL policy.


We directly follow SkilD \cite{pertsch2021guided}, to embed a sequence of $H$ consecutive actions $a_{0:H-1}$, known as a \textit{skill},  into a latent space using a variational autoencoder (VAE) \cite{kingma2013auto}. The VAE objective contains three parts: 1) a reconstruction loss to minimize the difference between demonstration actions $a_k$ and those predicted by the decoder $\hat{a}_k = g_{\psi_a}(a|s,z)$; 2) regularization on the encoder $q_\zeta(z|s_{0:H-1},a_{0:H-1})$ to align the latent distribution with a standard normal distribution; and 3) a KL-divergence term to train the skill prior $p_{\psi_z}(z|s_0)$ to match the  posterior distribution inferred from the encoder. The first two terms are standard components of a VAE \cite{kingma2013auto}, and the third term trains the skill prior that can accelerate downstream RL  \cite{pertsch2021accelerating}. We use a state-dependent decoder, $g_{\psi_a}(a|s,z)$ \cite{pertsch2021guided}, and augment the state with a one-hot vector corresponding to the time since skill selection for a more informative policy.
% Full training details are provided in Appendix \ref{Subsec:learn_skill}.

The skill prior parameterizes a Gaussian distribution and can be used directly to initialize and regularize a downstream HL policy \cite{pertsch2021accelerating, pertsch2021guided}.
In the next section, we extend this notion to an \textit{action prior} that can initialize and regularize a downstream LL policy.
% Then the HL and LL policy can be optimized in parallel. 
The pre-trained (deterministic) skill decoder is an obvious choice for the action prior, as previous works directly use the decoder as the LL policy  \cite{pertsch2021accelerating, pertsch2021guided}. Thus, we define a Gaussian action prior, denoted as $p_{\bar{\psi}_a}(a|z,s)=\mathcal{N}(\mu_{\hat{a}}, \sigma_{\hat{a}})$, with mean given by the skill decoder: $\mu_{\hat{a}}= g_{\psi_a}$. While the variance, $\sigma_{\hat{a}}$, is a hyperparameter we set, we note this action prior provides a more informative prior distribution than SAC's entropy term (unit Gaussian prior)\cite{pertsch2021accelerating}.  
% Appendix~\ref{Appendix: Ablation} studies the effect of $\sigma_{\hat{a}}$ on training performance. 


\subsection{Hierarchical Skill-Prior and Action-Prior Regularized RL Fine-tuning (Stage 2)}\label{Sec:HRLregularize}

\begin{algorithm}[b]
\caption{The Skill-Critic RL Algorithm} \label{Alg:skill-critic-summary}
\begin{algorithmic}[1]
% \renewcommand{\arraystretch}{2.0}
\STATE \textbf{Inputs:} Skill prior $p_{\psi_z}(z|s)$ and action prior $p_{\bar{\psi}_a}(a|s,z)$
%, initial network weights, hyperparameters
\FOR{each iteration}
\FOR{each environment step}
\IF{$t \mod H == 0$}
\STATE Sample skill $z\sim \pi_{\theta_z}(\cdot|s)$
\ENDIF
\STATE Sample action $a_t\sim \pi_{\theta_a}(\cdot|s_t,z)$
\STATE Perform action; add  $\{s,z,a,r,s'\}_t$ to replay buffer
\ENDFOR
\FOR{$t = 0,H, 2H,...$ and $t^*\doteq t+H$ }
\STATE Update HL policy, critic, and temperature towards Eqn.~\eqref{Eqn:HL obj} (i.e SPiRL \cite{pertsch2021accelerating})
\ENDFOR
\FOR{$t = 0,1,2,...$ and $t'\doteq t+1$}
\STATE Update LL policy, critic, and temperature towards Eqn.~\eqref{Eqn:LL obj}) via Algorithm~\ref{Alg:low-level})
\ENDFOR
\ENDFOR

\STATE \textbf{Return} trained HL policy $\pi_{\theta_z}$ and 
 LL policy $\pi_{\theta_a}$

\end{algorithmic}
\end{algorithm}

We now present Skill-Critic (Algorithm \ref{Alg:skill-critic-summary}),  which exploits a parallel MDP structure to optimize the HL and LL policy with guidance from the pre-trained skill prior and action prior. To derive our method for the parallel policy optimization of $\pi_a$ and $\pi_z$, we first note that learned skill space forms a semi-MDP endowed with skills in Section \ref{subsub:semiMDP}. This semi-MDP formulation can be written as parallel MDP formulation  (Section \ref{subsub:parallel}), so that we optimize the HL policy $\pi_{z}$ on a``high-MDP'' $M^\mathcal{H}$ and the LL policy $\pi_{a}$ on a ``low-MDP'' $M^\mathcal{L}$. Finally, in Sections \ref{subsub:high} and \ref{subsub:low}, the HL and LL policy optimizations are respectively guided by the pre-trained skill prior, $p_{\psi_z}(z|s)$, and action prior, $p_{\bar{\psi}_a}(a|s,z)$.  In each policy optimization problem, we initialize the trained policy with the corresponding pre-trained prior policy and augment the objective function with the KL divergence between the trained policy and its corresponding prior. 

 Our formulation makes three notable improvements on prior works: 1.) we employ a \textit{skill-based} parallel MDP formulation to update the HL and LL policies in parallel, 2.) we introduce a LL Q-function estimate using known relationships between state-action values on the MDPs  to stabilize optimization, and 3.) we extend soft actor-critic (SAC)~\cite{haarnoja2018soft} with non-uniform priors \cite{pertsch2021accelerating} to guide the LL policy update with the action prior.


\subsubsection{Semi-MDP endowed with skills}
\label{subsub:semiMDP}The hierarchical policies $\pi_a$ and $\pi_z$ form an MDP endowed with skills. We argue this is a semi-MDP similar to the one defined in the options framework \cite{sutton1999between}, as skills are continuous, fixed-duration options.
 The state space $\mathcal{S}$ consists of the environment states that are augmented with a one-hot encoding of the time index since the beginning of the active skill, $k_t \doteq (t \mod H )\in \mathcal{K}\doteq\{0,1,...H-1\}$. Following options notation \cite{zhang2019dac}, the skill can be defined as a triple $(\mathcal{I}, \pi_a, \beta)$, with initiation set $\mathcal{I}$, intra-skill policy $\pi_a:\mathcal{S}\times \mathcal{Z}\rightarrow \mathcal{A}$, and termination function $\beta: \mathcal{S}\rightarrow [0,1]$. In our case, we set $\mathcal{I}$ to the subset of states in $\mathcal{S}$ where $k=0$, so that skills are only initiated after a fixed horizon $H$ since the previous skill was initiated. The termination function is likewise  $\beta(s_t)\doteq\beta_t\doteq \mathbb{I}_{k_t=0}$, which takes value $\beta_t=1$ when $k_t=0$ and $\beta_t=0$ otherwise.
The semi-MDP consists of $M^\Omega \doteq \{\mathcal{S}, \mathcal{A}, \mathcal{Z}, R, p, p_0, \gamma\}$, of states, actions, skills,  reward, transition probability, initial state distribution, and
discount factor.  The RL objective, $\mathbb{E}_{\pi_a,\pi_z,\beta}[\Sigma_{t=0}^{T-1} \gamma^t r_t]$, maximizes the expected discounted rewards induced by $\pi_a$, $\pi_z$, and $\beta$.

The HL and LL value functions can be adapted from by option-critic~\cite{sutton1999between, bacon2017option} to continuous, fixed horizon skills:
\begin{equation}\label{eq:semiMDP}\begin{gathered}
V^\Omega_z\left( s_{t + 1} \right) = \mathbb{E}_{z_{t + 1}\sim\pi_{\theta_{z}}}\left\lbrack {Q_z^{\Omega}\left( {s_{t + 1},z_{t + 1}} \right) } \right\rbrack\\
Q^{\Omega}_z\left( {s_{t},z_{t}} \right) = \mathbb{E}_{a_{t}\sim\pi_{\theta_{a}}}\left\lbrack {Q^{\Omega}_a\left( {s_{t},z_{t},a_{t}} \right) } \right\rbrack\\
Q^{\Omega}_a\left( {s_{t},z_{t},a_{t}} \right) = r\left( {s_{t},a_{t}} \right) + \gamma\mathbb{E}_{a_{t + 1}\sim\pi_{\theta_{a}},\pi_{\theta_{z}}}\left\lbrack {U\left( {z_{t},s_{t + 1}} \right)} \right\rbrack\\
U\left( {z_{t},s_{t + 1}} \right) = \left\lbrack {1 - \beta_{t + 1}} \right\rbrack Q^{\Omega}_z\left( {s_{t + 1},z_{t}} \right) +\beta_{t + 1} V^{\Omega}_z\left( s_{t + 1} \right).
\end{gathered}
\end{equation}
Here $V^\Omega_z$ is the value of the state $s_t$, $Q_z^\Omega$ is the value of selecting skill $z_t$ from $s_t$, and $Q^\Omega_a$ is the value of selecting action $a_t$ from state $s_t$ and skill $z_t$.
Simplifying for fixed horizon skills, when $\beta(s_{t+1})=0$ during rollout of a skill,
\begin{equation}\label{Eqn: Qa_noreg_b0}
\begin{gathered}
    Q^\Omega_{a, \beta_{t+1}=0} = r(s_t,a)+\mathbb{E}_{\pi_a,\pi_z}[Q^\Omega_a(s_{t+1},z_{t+1},a_{t+1})].
    \end{gathered}
\end{equation}
and when $\beta(s_{t+1})=1$ at selection of the next skill
\begin{equation}\label{Eqn: Qa_noreg_b1}
            Q^\Omega_{a, \beta_{t+1}=1} = r(s_t,a)+\mathbb{E}_{\pi_a,\pi_z}[Q^\Omega_z(s_{t+1},z_{t+1})].
\end{equation}





\subsubsection{Formulation as two augmented MDPs} \label{subsub:parallel}
The above semi-MDP formulation requires special algorithms to solve \eqref{eq:semiMDP}\cite{bacon2017option}, which are difficult to augment with skill and action prior regularization. 
Therefore, we formulate the semi-MDP as two parallel augmented MDPs, so that any off-the-shelf policy optimization algorithms can be used to learn each policy \cite{zhang2019dac}. We adapt an options-based parallel MDP framework, Double Actor Critic (DAC) \cite{zhang2019dac}, to our continuous, fixed-horizon skills.
The HL policy $\pi_z$ makes decisions (selects skills) in the high-MDP $M^\mathcal{H}$, and the LL policy $\pi_a$ makes  decisions (selects actions) in the low-MDP $M^\mathcal{L}$.

We define $p_z$ as the transition probability function from the current state and skill to the next state:
\begin{equation}\label{eq:skill_transition_function}
    p_z\left(s_{t+1} | s_t, z_t\right)\doteq \mathbb{E}_{ a\sim \pi_{a}\left(a | s_t, z_t\right)} \left[p\left(s_{t+1} | s_t, a\right)\right].
\end{equation}
Eq. \ref{eq:skill_transition_function} is analogous to the first equation in Section 2 of DAC \cite{zhang2019dac}; however, we directly define $p_z$ by taking the expectation over actions instead of using a discrete probabilistic estimate. Similarly, we define the skill-based reward function as 
\begin{equation}
    r_z\left(s_t, z_t\right)\doteq \mathbb{E}_{ a_t\sim \pi_{a}\left(a \mid s_t, z_t\right)} \left[r\left(s_t,  a_t\right)\right].
\end{equation}


  
% \begin{equation}
%     r_z\left(s_t, z_t\right)\doteq \mathbb{E}_{ a_t\sim \pi_{a}\left(a \mid s_t, z_t\right)} \left[r\left(s_t,  a_t\right)\right].
% \end{equation}
For the remainder of the derivation, we use an almost identical notation to DAC, Section 3 \cite{zhang2019dac}; the only change is that we replace the discrete options, $O\sim \mathcal{O}$, with skills, $Z\sim \mathcal{Z}$, and adjust the equations accordingly.
 To form the high-MDP $M^\mathcal{H}$, the state is composed of the current state and skill $S_{t}^\mathcal{H}\doteq (z_{t-1}, s_t)$, and the action is the next skill $A^\mathcal{H}\doteq z_t$. Thus, we can write $M^{\mathcal{H}}$ as a regular MDP:
\begin{equation}
        \begin{aligned}
        & 
        \mathcal{S}^{\mathcal{H}} \doteq  \mathcal{Z}\times\mathcal{S}, \quad \mathcal{A}^{\mathcal{H}} \doteq \mathcal{Z} \\ 
M^{\mathcal{H}} & \doteq\left\{\mathcal{S}^{\mathcal{H}}, \mathcal{A}^{\mathcal{H}}, p^{\mathcal{H}}, p_0^{\mathcal{H}}, r^{\mathcal{H}}, \gamma\right\},  \\
p^{\mathcal{H}}\left(S_{t+1}^{\mathcal{H}} \mid S_t^{\mathcal{H}}, A_t^{\mathcal{H}}\right) & \left. \doteq p^{\mathcal{H}}\left( (z_t,s_{t+1}) \mid (z_{t-1},s_t), A_t^{\mathcal{H}}\right)\right) \\ & \doteq \mathbb{I}_{A_t^{\mathcal{H}}=z_t} p_z\left(s_{t+1
} \mid s_t, z_t\right) \\ 
p_0^{\mathcal{H}}\left(S_0^{\mathcal{H}}\right) & \doteq p_0^{\mathcal{H}}\left((z_{-1},s_0)\right)  \doteq p_0\left(s_0\right), \\ 
r^{\mathcal{H}}\left(S_t^{\mathcal{H}}, A_t^{\mathcal{H}}\right) & \doteq r^{\mathcal{H}}\left((z_{t-1}, s_t), z_t\right) \doteq r_z\left(s_t, z_t\right), 
\end{aligned}
\end{equation}
where $\mathbb{I}$ is the indicator function. It is not necessary to define a dummy skill \cite{zhang2019dac}, since we always start with skill selection from policy $\pi_z(z_t|s_t)$ at $t=0$. 

We define the Markov policy $\pi^\mathcal{H}$ on $M^\mathcal{H}$ as 
\begin{equation}\label{Eqn: pi_H}
\begin{aligned}
    \pi^{\mathcal{H}}\left(A_t^{\mathcal{H}} \mid S_t^{\mathcal{H}}\right) & \doteq \pi^{\mathcal{H}}\left(z_t \mid (z_{t-1}, s_t)\right) \\ \doteq (1&-\beta(s_t)) \mathbb{I}_{z_{t-1}=z_t} + \beta(s_t)\pi_z \left(z_t \mid s_t\right).
    \end{aligned}
\end{equation}
Eq.~\eqref{Eqn: pi_H}  shows that the previous skill is used until  $\beta(s_t)=1$; then a new skill is selected via $\pi_z$. 
It is similar to the definition in DAC \cite{zhang2019dac}; however, we can exploit the definition of $\beta$ to reduce \eqref{Eqn: pi_H} to only be a function of $\pi_z$ and $\beta$. 




In the low-MDP, $M^\mathcal{L}$, the state is composed of the current state and next skill, $S_{t}^\mathcal{L}\doteq (s_t, z_t)$, and the action is the action $A^\mathcal{L}\doteq a_t$.
 Then $M^{\mathcal{L}}$ is the regular MDP
\begin{equation}
\begin{aligned}
\mathcal{S}^{\mathcal{L}} & \doteq \mathcal{S} \times \mathcal{Z}, \quad \mathcal{A}^{\mathcal{L}} \doteq \mathcal{A} \\ 
    M^{\mathcal{L}} & \doteq\left\{\mathcal{S}^{\mathcal{L}}, \mathcal{A}^{\mathcal{L}}, p^{\mathcal{L}}, p_0^{\mathcal{L}}, r^{\mathcal{L}}, \gamma\right\} \\
p^{\mathcal{L}}\left(S_{t+1}^{\mathcal{L}} \mid S_t^{\mathcal{L}}, A_t^{\mathcal{L}}\right) & \doteq p^{\mathcal{L}}\left(\left(s_{t+1}, z_{t+1}\right) \mid\left(s_t, z_t\right), a_t\right) \\ &\doteq p\left(s_{t+1} \mid s_t, a_t\right) p\left(z_{t+1} \mid s_{t+1}, z_t\right) \\
p_0^{\mathcal{L}}\left(S_0^{\mathcal{L}}\right) & \doteq p^{\mathcal{L}}\left(\left(s_0, z_0\right)\right)  \doteq  \pi_z\left(z_0|s_0\right)p_0\left(s_0\right) \\ 
r^{\mathcal{L}}\left(S_t^{\mathcal{L}}, A_t^{\mathcal{L}}\right) & \doteq r^{\mathcal{L}}\left(\left(s_t, z_t\right), a_t\right)  \doteq r\left(s_t, a_t\right).
\end{aligned}
\end{equation}
We define a Markov policy $\pi^\mathcal{L}$ on $M^\mathcal{L}$ as the LL policy $\pi_a$:
\begin{equation}
    \pi^{\mathcal{L}}\left(A_t^{\mathcal{L}} \mid S_t^{\mathcal{L}}\right) \doteq \pi^{\mathcal{L}}\left(a_t \mid\left(s_t, z_t\right)\right) \doteq \pi_{a}\left(a_t \mid s_t,z_t\right).
\end{equation}
It follows that when we fix  $\pi_a$ and optimize $\pi^\mathcal{H}$, we are optimizing $\pi_z$. Likewise, when we fix $\pi_z$ and optimize $\pi^\mathcal{L}$, we are optimizing $\pi_a$~\cite{zhang2019dac}. This implies that any policy optimization algorithm can be used to optimize $\pi^\mathcal{H}$ and $\pi^\mathcal{L}$.



% \clearpage
\subsubsection{High-MDP Policy Optimization} \label{subsub:high} To optimize $\pi^\mathcal{H}$ on $M^\mathcal{H}$, policy $\pi_{z}$ is parameterized by $\theta_z$ (denoted $\pi_{\theta_z}$), and we fix $\pi^\mathcal{L}$. The skill prior, $p_{\psi_z}$, is a prior distribution for $\pi_{\theta_z}$, and $\theta_z$ is initialized with $\psi_z$. 
The \textit{HL update} in Fig.~\ref{fig:framework} solves 
\begin{equation}
\label{Eqn:HL obj}
\begin{aligned}
\underset{\theta_z}{\operatorname{argmax}} \;\mathbb{E} _{\pi_{\theta_z},\pi^\mathcal{L}}&\left[\sum_{t=\{0, H, 2H, \hdots \}}^{\infty} \gamma_z^t \Big(\tilde{r}_H(s_t, z_t) \right. \\
& \left. -\alpha_z D_{K L}[\pi_{\theta_z}(z_t | s_t) \| p_{\psi_z}(z_t | s_t)]\Big)\right].
\end{aligned}
\end{equation}
where the regularization term is weighted with temperature $\alpha_z$.
Since $\pi^\mathcal{H}$ executes a skill for $H$ time steps, at which point $\pi_{\theta_z}$ selects a new skill, we employ an $H$-step reward:  $\tilde{r}_H(s_t,z_t) := \Sigma_{\tau = t}^{t+H-1} r(s_\tau, a_\tau)$.  The RL objective is valid since for fixed-horizon skills, $M^\mathcal{H}$ can be represented with $r^\mathcal{H}\doteq \tilde{r}_H$ when evaluated only at instances when the skills change ($\beta(s)=1$) \cite{pertsch2021accelerating}. We solve \eqref{Eqn:HL obj} using the Bellman operator on $M^\mathcal{H}$:
\begin{equation}\label{Eqn: spirl_bellman}
    \begin{aligned}
        &\mathcal{T}^{\pi_z} Q^\mathcal{H}\left(s_t, z_t\right)=\tilde{r}_H\left(s_t, z_t\right)+\gamma \mathbb{E}_{p^{\mathcal{H}}}\left[V^\mathcal{H}\left(s_{t+1}\right)\right]\\
         &V^\mathcal{H}\left(s_t\right)=\mathbb{E}_{z_t \sim \pi_z}\big[Q^\mathcal{H}\left(s_t, z_t\right) \\& \qquad \qquad \qquad-D_{\mathrm{KL}}\left[\pi_z\left(z_t | s_t\right) \| p_{\psi_z}\left(z_t |s_t\right)\right]\big].
    \end{aligned}
\end{equation}
The value function $V^\mathcal{H}$ and Q-function $Q^\mathcal{H}$ are defined on $M^\mathcal{H}$ using the Bellman operator in SPiRL \cite{pertsch2021accelerating}, which is proven to solve \eqref{Eqn:HL obj} by adapting SAC \cite{haarnoja2018soft}. 
This $H$-step reward, $\tilde{r}_H$, implies that the state-skill value estimation in the HL Q-value, $Q^\mathcal{H}(S_t^\mathcal{H}, A_t^\mathcal{H})\doteq Q^z(s_t,z_t)$ is discounted every $H$ steps, which has improved performance on long-horizon tasks by increasing the effect of the sparse reward \cite{pertsch2021accelerating}.


\begin{algorithm}[b] 
\caption{Skill-Critic Low-MDP Update} \label{Alg:low-level}
\begin{algorithmic}[1]
% \renewcommand{\arraystretch}{2.0}
\STATE \textbf{Inputs: } Current iteration's HL parameters: $\bar{\phi}_z, \theta_z$; priors $p_z, p_\psi$, hyperparameters
\FOR{each $t = 0,1,2,...$ and $t'=t+1$ in replay buffer}
\IF{$k_{t}==H-1, \quad$ (where $k_{t}= t\mod H$)}
\STATE $\bar{Q}_{a} = Q^a_{\beta(s')=1}(s, z, a)$ using $Q_{\bar{\phi}_z}$ in \eqref{Eqn: Qat} \\ \COMMENT{Estimate LL Q-value  \textit{upon arrival} to new skill} \label{line:new_skill}
\ELSE
\STATE $\bar{Q}_{a} = Q^a_{\beta(s')=0}(s, z, a)$ using $Q_{\bar{\phi}_a}$ in \eqref{Eqn: Qatau} \\ \COMMENT{Estimate LL Q-value  within current skill}
\ENDIF
\STATE $\theta_{a}\leftarrow $ step on \eqref{Eqn:LL obj} using $Q_{\phi_a}$ \COMMENT{update LL policy parameters}
\STATE $\phi_{a} \leftarrow \phi_{a} - \lambda_{Q_a} \nabla_{\phi_{a}} [\frac{1}{2} ( Q_{\phi_a}\left(s_{t},a_t, z_t\right) - \bar{Q}_a )^2 ]$ \\ \COMMENT{update LL critic weights}
\STATE $\alpha_a \leftarrow \lambda_{\alpha_a}\big[\alpha_a( D_{KL}(\pi_{\theta_a}(a_t|s_t,z_t)\| p_{\bar{\psi}_a}(a_t|s_t,z_t))  - \delta_a)\big]$ \\ \COMMENT{update LL alpha} 
\STATE $\bar{\phi}_a \leftarrow \tau \phi_a + (1-\tau)\bar{\phi}_a$  \COMMENT{update LL target network weights}
\ENDFOR
\STATE \textbf{Return} trained low-level policy $\pi_{\theta_a}$
\end{algorithmic}
\end{algorithm}


\subsubsection{Low-MDP Policy Optimization}\label{subsub:low} To optimize $\pi^\mathcal{L}$ on $M^\mathcal{L}$, policy $\pi_{a}$ is parameterized by $\theta_a$ (denoted $\pi_{\theta_a}$), and we fix $\pi^\mathcal{H}$. The action prior learned from offline demonstrations, $p_{\bar{\psi}_a}$, is a prior distribution for $\pi_{\theta_a}$, and $\theta_a$ is initialized with $\bar{\psi}_a$. The regularized objective with temperature $\alpha_a$ is
\begin{equation} \label{Eqn:LL obj}
\begin{aligned}
\underset{\theta_a}{\operatorname{argmax}} \; &\mathbb{E}_{\pi_{\theta_a}, \pi^\mathcal{H}}\left[\sum_{t=0}^{\infty} \gamma^t_a \Big(r\left(s_t, a_t\right) \right. \\
& \left. -\alpha_a D_{K L}\left[\pi_{\theta_a} (a_{t} | s_{t}, z_t) \| p_{\bar{\psi}_a}(a_{t}  | s_{t}, z_t, )\right]\Big)\right].
\end{aligned}
\end{equation}
Eq.~\eqref{Eqn:LL obj} corresponds to the \bluetext{\textit{LL update}} in Fig.~\ref{fig:framework}. We employ the LL update in Algorithm~\ref{Alg:low-level}, which adapts  KL-divergence regularized SAC to solve \eqref{Eqn:LL obj}. First, we define the following Bellman operator on $M^\mathcal{L}$:
\begin{equation}\label{Eqn: ll_bellman}
    \begin{aligned}
       & \mathcal{T}^{\pi_a} Q^\mathcal{L}\left((s_t,z_t), a_t\right)=r\left(s_t, a_t\right)+\gamma \mathbb{E}_{p^\mathcal{L}}\left[V^\mathcal{L}\left((s_{t+1},z_{t+1})\right)\right]\\
        &V^\mathcal{L}\left((s_t,z_t)\right)=\mathbb{E}_{a_t \sim \pi_{a}}\big[Q^\mathcal{L}\left((s_t,z_t), a_t\right)\\ & \qquad \qquad -D_{\mathrm{KL}}\left[\pi_a\left(a_t | (s_t,z_t)\right) \| p_{\bar{\psi}_a}\left(a_t | (s_t,z_t)\right)\right]\big].
    \end{aligned}
\end{equation}
% We apply the same a variant of SAC as the HL update \cite{pertsch2021accelerating} to Eqn. \eqref{Eqn:LL obj} to perform the LL update in Algorithm~\ref{Alg:low-level}. 
Similar to the HL update, the entropy regularization in SAC is replaced with  the deviation of the policy $\pi_{\theta_a}$ from the prior $p_{\bar{\psi}_z}$. Dual gradient descent on the temperature $\alpha_a$ \cite{haarnoja2018soft, pertsch2021accelerating} ensures that the expected divergence between LL policy and
the action prior is equal to the chosen target divergence $\delta_a$ on Line 9. 
The LL Q-value,
$Q^\mathcal{L}(S^\mathcal{L},A^\mathcal{L})\doteq Q^a(s,z,a),
$ estimates the value of the state-skill pair and action using 1-step exponential discounting  \eqref{Eqn:LL obj}.



When estimating $Q^a$ with \eqref{Eqn: ll_bellman}, far-horizon rewards have an exponentially diminishing effect. Practically,  this led to poor performance in sparse reward environments. 
Inspired by the relationship between Q-functions on the semi-MDP \eqref{eq:semiMDP}, we investigate if the longer-horizon HL Q-value can inform LL policy optimization of the value that the HL policy is assigning to state-skill pairs, thus allowing sparse rewards to propagate to earlier states. We observe in the semi-MDP formulation that $V_z^\Omega$ is analogous to the value of skills, meaning $V_z^\Omega$ is analogous to the value function on the high-MDP, $V^\mathcal{H}$. Likewise, $Q^\Omega_z$ is analogous to the value of state-skill pairs, meaning $Q^\Omega_z$ is analogous to the value function on the low-MDP, $V^\mathcal{L}$. 



The semi-MDP \eqref{eq:semiMDP} does not include policy regularization. To incorporate our non-uniform prior into $Q_a$ estimation, we note that the regularization terms in \eqref{Eqn: spirl_bellman} and \eqref{Eqn: ll_bellman} appear  in the definition of $V^\mathcal{H}$ and $V^\mathcal{L}$. 
We follow this precedent as we introduce regularization into \eqref{Eqn: Qa_noreg_b0}  and \eqref{Eqn: Qa_noreg_b1}.
We define
\begin{equation} \label{Eqn: Qat}
\begin{aligned}
Q^a_{\beta(s_{t+1})=1}\left(s_{t}, z_{t}, a_{t}\right)= & r\left(s_t, a_t\right)+\gamma \mathbb{E}_{\pi_z}\big[Q^z\left(s_{t+1}, z_{t+1}\right)\\
-\alpha_z D_{K L} & [\pi_{\theta_z}(z_t | s_t) \| p_{\psi_z}(z_t | s_t)] \big],
\end{aligned}
\end{equation}
 to  estimate $Q^a$ at the start of a new skill (Line 4, Alg. \ref{Alg:low-level}) and
\begin{equation} \label{Eqn: Qatau}
\begin{aligned}
 Q^a \left(s_{t}, z_t, a_{t}\right)= & r(s_t,a_t)+\gamma \mathbb{E}_{\pi_a, \pi_z}\big[Q^a(s_{t+1},z_{t+1},a_{t+1}) \\
-\alpha_a D_{K L} & \left[\pi_{\theta_a} (a_{t} | s_{t}, z_t) \| p_{\bar{\psi}_a}(a_{t}  | s_{t}, z_t, )\right] \big], \\
\end{aligned}
\end{equation}
 to  estimate $Q^a$ otherwise. While the semi-MDP assumptions do strictly hold for the regularized objective \eqref{Eqn:LL obj}, we find that using $Q^z$ to estimate $Q^a$ leads to faster, stable convergence. 
 
% Equation~\eqref{Eqn: Qat} is inspired by the relationship between Q-functions between Q-functions on the semi-MDP \eqref{Eqn: Qa_noreg_b0} and \eqref{Eqn: Qa_noreg_b1}.  


% \subsubsection{Skill-Critic} %\label{subsec:skillcriticalgo}
% The complete algorithm is summarized in Algorithm~\ref{Alg:skill-critic-summary}.
% After a skill embedding and prior are learned from demonstrations (Section~\ref{Sec:skillprior}), Skill-Critic uses the incomplete skill set to train the HL and LL policies. 
% Rollouts are collected from the environment by sampling the HL policy every $H$ steps, and executing the selected skill for $H$ steps by sampling the LL policy.
% The action is executed in the environment, and $\{s,z,a,r,s'\}$ is stored. 
% Policy improvement occurs in two stages. 
% The HL policy, $\pi_z$ is optimized on $M^\mathcal{H}$ using critics $Q_{\phi_z}$ and $Q_{\bar{\phi}_z}$, and temperature parameter $\alpha_z$ (Line 9) via SPiRL~\cite{pertsch2021accelerating}. The LL policy, $\pi_a$, is optimized on $M^\mathcal{L}$ using critics $Q_{\phi_a}$ and $Q_{\bar{\phi}_a}$, and $\alpha_a$ (Line 11) via Algorithm~\ref{Alg:low-level}. 

% Unlike previous works that fixed the LL policy during training (i.e. $\pi^\mathcal{L}\doteq p_{\bar{\psi}_a}$) \cite{pertsch2021accelerating}, the RL fine-tuning of $\pi^\mathcal{L}=\pi_{\theta_a}$ with initial policy $\pi_{\theta_a}^0=p_{\bar{\psi}_a}$ allows us to \textit{improve} skills to maximize rewards. 

% \subsection{Skill Discovery} \label{Subsec: SkillDisc}
% \commentc{I think this can be moved to the appendix. it is an implementation detail. Also I would not say you "add"  a variance head, because really you are just initializing a stochastic policy's weights with the  weights of the decoder, right?}
% The Skill-Critic agent discovers new skills by exploring and updating low-level action policies. However, the low-level policy has the same structure as the decoder and only outputs deterministic actions, limiting exploration efficiency. To this end, we adopt a common strategy for continuous action exploration \textemdash probabilistic policy with variance. We add another variance head to the policy network to simultaneously generate the mean and standard deviation $\{\mu, \sigma \} \sim \pi^a_{\phi}$ and formulate them to a Gaussian distribution $\mathcal{N}(\mu, \sigma)$. We manually initialize the value of the variance head $\sigma_0$ to keep a moderate speed of skill exploration and update.

% \begin{equation} \label{Eqn: DKL_LL}
%     D_{K L}  \left(\pi^a_{\phi}\left(a_{t} \mid s_{t}, z_i, \bar{k}_{t}\right) \|  p_\phi\left(\hat{a}_{t} \mid s_{t}, z_i, \bar{k}_{t}\right)\right)  = D_{K L}\left( \mathcal{N}( \mu_{t}, \sigma_t ) \| \mathcal{N}(\hat{\mu}_{t} ,\sigma_0) \right)
% \end{equation}

% In Eqn.~\eqref{Eqn:LL obj}, the KL divergence of low-level policy constraints the distribution difference with the decoder. In practice, we also consider the variance head and derive the calculation in Eqn.~\eqref{Eqn: DKL_LL}, where $\{\mu_{t}, \sigma_t\}$ are output from the mean and variance heads of the policy network, while only the mean $\hat{\mu}_{t}$ is output by the decoder network and the variance $\sigma_0$ is still the initial value. So we constrain the low-level policy with the decoder output and the expected variance. We control the magnitude of KL divergence by setting a target value $\delta$ and use an auto-tuning strategy in (ref SPiRL) to regularize $\alpha$ and guide the policy convergence.





==> submit1/submittedRAL/conclusion.tex <==
% ============== conclusion =============
\section{Conclusion} \label{Sec:Conclusion}
We proposed Skill-Critic, a hierarchical skill-transfer RL algorithm, to perform two parallel policy optimization updates for skill selection and skill fine-tuning. We show that Skill-Critic can effectively leverage low-coverage and low-quality demonstrations to accelerate RL training, which is difficult with existing skill-transfer RL methods with stationary LL policies. In our experiments, our method can solve maze navigation tasks that require exploring new skills in online fine-tuning. Furthermore, Skill-Critic can solve a challenging sparse-reward autonomous racing task with the help of low-quality, non-expert demonstrations. Finally, Skill-Critic learns to perform robotic manipulation task faster than existing hierarchical RL methods.


\textit{Limitations and Future Work:} Skill-Critic reformulates  hierarchical RL as two parallel MDPs. Alternating between HL and LL policy optimization does not guarantee an optimal joint policy for the original semi-MDP. In future work, we are interested in alternative theoretical frameworks where the HL and LL policies are jointly optimized for a single KL-regularized semi-MDP. Furthermore, we plan to alleviate the restriction of fixed skill horizons with adaptive skill horizons. 


==> submit1/submittedRAL/experiments.tex <==

% =============== experiments ===========
\section{Experiments} \label{Sec:Exp}
% Our experiments aim to answer: (1) Can Skill-Critic effectively leverage low-coverage, low-quality demonstrations to accelerate downstream RL? (2) Is the proposed LL policy update step necessary in improving the skill set and optimizing the agent performance in the downstream task?  

 We assess Skill-Critic in three tasks: maze navigation, vehicle racing, and robotic manipulation.  For each environment, Stage 1 consists of collecting a large, offline dataset to create an informative skill set; however, the skill set may not encompass \textit{all} of the potential skills that aid downstream tasks. Stage 2 consists of a  sparse-reward episodic RL task; specifically, a binary reward (+1) is received at each time step after the goal is reached. The objective is to maximize the sum of rewards, i.e. complete the task \textit{as fast as possible}.

 % We evaluate the environment reward, to test not only whether the task is completed, but also how well the task is completed. 


\subsection{Maze Navigation and Trajectory Planning}
We employ a maze-based task to examine if Skill-Critic can simultaneously improve its LL policy and  leverage the offline action prior to learn challenging, long-horizon tasks.
The maze task is based on the D4RL point maze environment~\cite{fu2020d4rl} that uses a top-down agent-centric state and continuous 2D velocity as the action. Demonstrations consist of 85000 goal-reaching trajectories in randomly generated, small maze layouts in Fig.~\ref{fig:env_maze}. The demonstration planner~\cite{pertsch2021accelerating} plans actions in right angles (i.e. the demonstrator goes straight up/down or left/right). In Stage 1, the agent can learn skills such as traversing hallways or passing through doors.
% that it can transfer to Stage 2. 

For Stage 2 downstream learning, we introduce two new maze layouts: 1.) a \textit{Diagonal Maze} to test how well the agent can navigate a maze with unseen passageways, and 2.) a \textit{Curvy Tunnel} with multiple options for position, heading, and velocity to test how well the agent can plan an optimal trajectory. In both layouts, the agent has 2000 steps in each episode and receives a binary reward for each time step that the distance to the goal is below a threshold. Unlike the downstream tasks in SPiRL \cite{pertsch2021accelerating}, in the maze layouts we introduce, the agent can significantly improve its performance by moving diagonally and following a smooth, optimal path.
\begin{figure}[t]
    \centering
    \includegraphics[width=.27\textwidth,trim={0 0pt 0 0pt},clip]{figures/env1_cropped.pdf}
    \caption{Maze Tasks. Stage 1 demonstration uses the planner in SPiRL \cite{pertsch2021accelerating}. We create two complicated stage 2 RL tasks to test the agent's navigation in a \textit{Diagonal Maze} (left) and path planning in a \textit{Curvy Tunnel} (right).}
    \label{fig:env_maze}
\end{figure}

We aim to test whether Skill-Critic can accelerate downstream RL using offline demonstrations and improve task performance with the LL policy update. We compare Skill-Critic to several baselines in Fig.~\ref{fig:MazeResults}.\textbf{SPiRL}~\cite{pertsch2021accelerating} extracts temporally extended skills with a skill prior from the offline data, but downstream RL training occurs only on the HL skill selection policy. Our version of SPiRL uses a state-dependent policy to improve performance~\cite{pertsch2021guided}. \textbf{Skill-Critic} is warm-started with SPiRL at 1M steps to stabilize the HL policy prior to LL policy improvement.
Additional baselines include soft actor-critic (\textbf{SAC})\cite{haarnoja2018soft} and a policy initialized with behavioral cloning and fine-tuned with SAC (\textbf{BC+SAC}). 

In both tasks, SAC and BC+SAC fail to reach the goal, likely because the single-step policy is unable to discover the sparse reward. In comparison, the temporally abstracted methods (SPiRL and Skill-Critic) can effectively utilize offline demonstrations to successfully reach the goal. We compare the trajectories of Skill-Critic and SPiRL in the right of Fig. \ref{fig:MazeResults}. SPiRL plans slow, jagged trajectories because it cannot improve the offline-learned skills to further improve reward.   Skill-Critic is able to update the LL policies and further optimize its path, resulting in planning a significantly faster trajectory.  Interestingly, Skill-Critic \textit{discovers} diagonal motion, but it still does not forget to solve the maze because LL policy exploration is guided by the action prior.
% (see ablations in Section \ref{subsec: ablation}).
% (ablations in Appendix~\ref{Appendix: Ablation}).

\begin{figure*}[t]
    \centering
        \includegraphics[width=0.32\textwidth]{figures/maze.pdf}
    \includegraphics[width=0.30\textwidth,trim={25cm 0 0 0},clip]{figures/MazeExp.pdf}
    \caption{Maze task results. \textbf{Left:} mean (std) episode rewards with 3 random seeds. Skill-Critic begins training at 1 million steps and is warm-started by SPiRL.\textbf{Right:} Trajectories after policies converge. SPiRL reuses right-angle skills, but Skill-Critic discovers new skills to plan  diagonal and curved paths.}
    \label{fig:MazeResults}
\end{figure*}





\subsection{Autonomous Racing}
The vehicle racing task tests if Skill-Critic can 1.) improve the LL policy when there is only access to low-coverage, low-quality demonstrations, and 2.) leverage the skill and action prior to accelerate learning of a long-horizon sparse reward.
We employ the Gran Turismo Sport (GTS) high-fidelity racing simulator to solve a new, sparse reward autonomous racing task. The low-dimensional state representation \cite{fuchs2021super} includes pose, velocity, and track information. There are two continuous actions: steering angle and a combined throttle/brake command between $[-1,1]$. 
Unlike previous works in GTS with dense rewards that must be hand-designed for each car and track~\cite{fuchs2021super, wurman2022outracing}, we create a generalizable sparse reward in a single corner (Fig.~\ref{fig:env_racing}). The agent starts at a low speed in the center of the track and has 600-step (60-sec) episodes; the agent receives a binary +1 reward at each time step after it passes the goal.  

We use GTS's built-in AI controller to collect 40000 \textit{low-speed} demonstrations from random starting points on the course, each 200 steps in length. While the built-in AI is capable of controlling the race car at high speed, to collect the dataset, we deliberately start at low initial speeds to test Skill-Critic's ability to improve skills. The agent can transfer skills such as speeding up and turning, but must learn to drive the vehicle at higher speeds to rapidly navigate the corner.%as fast as possible.

We evaluate Skill-Critic with the same baseline policies as the maze task and also consider GTS's Built-in AI as a strong baseline. The Built-in AI is a high-quality, rule-based controller deployed with the game as a competitor for players. Note that the policies only have access to short horizon, low-speed demonstrations from the Built-in AI, and the long-horizon, sparse reward task is much harder than maximizing hand-engineered dense rewards~\cite{wurman2022outracing}. 
In Fig.~\ref{fig:RaceResults}, we evaluate two signals over the course of training: episode rewards, which increase when the car completes the course faster, and time in contact with the wall at the edge of the track, which indicates the car's dynamic stability.
We compare  trajectories from each method's highest reward policy. 



None of the baseline policies are able to efficiently solve the sparse-reward racing. SAC reaches the goal in spite of its single-step policy, but it is slow to improve with the sparse reward; thus policies have relatively low velocity. Warm-starting the SAC policy appears to hinder exploration; in fact, BC+SAC fails to reach the goal, consistently crashing within the first straight-away when the policy visits states unseen in the demonstrations.
In contrast, SPiRL exploits the pre-trained skills to consistently reach the goal. However, these skills are learned from low-speed demonstrations, and the environment has complex vehicle dynamics. Thus, SPiRL's HL policy cannot generate high-speed trajectories from the stationary LL policy, which may only be capable of low-speed maneuvers. SPiRL's stationary LL policy may suffer from distributional shifts if the demonstrations are not sufficient to cover the vehicle dynamics at unseen states. Thus, SPiRL is unable to improve its policy and often collides with the wall.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.25\textwidth]{figures/env2_cropped.pdf}
    \caption{Vehicle racing task. The course consists of a corner, and the agent achieves a sparse reward after the goal state is passed.  Demonstrations are collected at random low-speed starting points on the course. }
    \label{fig:env_racing}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figures/gts_no_traj.pdf}    \caption{Vehicle racing results. \textbf{Left:} mean (std) episode reward. \textbf{Right:} mean (std) of cumulative time in contact with track boundary wall per episode. }
    \label{fig:RaceResults}
\end{figure}
Skill-Critic addresses these issues to achieve higher episode rewards, reduce contact time with course walls, and quickly navigate the corner. Skill-Critic exploits the offline pre-training and temporally extended actions to guide exploration. Notably, the online LL fine-tuning allows Skill-Critic to learn high velocity maneuvers, such as collision avoidance and sharp cornering.   Despite the sparse reward and low-speed demonstrations, Skill-Critic is the only learned policy that can consistently perform as well as the Built-in AI.
\begin{figure}[t]
    \centering
    \includegraphics[width=.25\textwidth]{figures/env3_cropped.pdf}
    \caption{Robotic task. Stage 1 demonstrations use the planner in ReSkill \cite{rana2023residual} to push a block across a table. Stage 2 RL tasks are \textit{Slippery Push}, which alters the coefficient of friction to make a more slippery surface, and \textit{Table Cleanup}, which includes a tray as an obstacle for the robot's task. }
    \label{fig:env_robot}
\end{figure}
\begin{figure}[t]
    \centering
        \subfigure[Table Cleanup]{
    \includegraphics[width=.46\columnwidth]{figures/cleantable.pdf}}
            \subfigure[Slippery Push]{
    \includegraphics[width=.46\columnwidth]{figures/slippery_rew.pdf}}
    \caption{\textbf{\color{black}{Evaluation on 7DoF Robotic Arm. }} \color{black}{Mean episode reward (std) for each environment. Skill-Critic is warm-started with SPiRL at 500k steps.  }}
    \label{fig:fetchresults}
\end{figure}

\subsection{Robot Manipulation}  We implement an armed robot experiment to evaluate how well Skill-Critic performs in comparison to existing hierarchical RL methods on sparse reward manipulation tasks. The environment is a 7-DoF Fetch robotic arm simulated in MuJoCO \cite{todorov2012mujoco}. The demonstration environment is a \textit{Push} task were the robot must push a block along a table (Fig.~\ref{fig:env_robot}). The handcrafted controllers in Rana et al. \cite{rana2023residual} collected 40k demonstration trajectories. 
For the Stage 2 RL tasks, we employ a \textit{Slippery Push} and \textit{Table Cleanup} task \cite{rana2023residual}.
The \emph{Slippery Push} the agent must push a block to a goal, but the friction of the table surface is lowered from that seen in the demonstrations. The agent receives a reward of 1 once the block is at the goal location, otherwise the reward is 0. The task is episodic and terminates after 100 steps. 
For \emph{Table Cleanup} task, the agent must place a block on a rigid tray object, which was not present in the demonstrations. The agent receives a reward of 1 only when the block is placed on the tray, otherwise the reward is 0. The task is episodic and terminates after 50 steps. 



In addition to SPiRL \cite{pertsch2021accelerating}, we test 
\textbf{ReSkill}~\cite{rana2023residual}, a hierarchical RL method that uses residual skill policies to augment the stationary LL policy during training. This is in contrast to Skill-Critic, which directly fine-tunes the non-stationary LL policy with regularization to the stationary action prior.
  In ReSkill, the HL and LL policy optimizations are iterative and completely independent. In contrast, our proposed Skill-Critic algorithm exploits the relationship between the HL and LL policies to relate the LL Q-function to the HL Q-function upon arrival at the next skill (Eq. \ref{Eqn: Qatau} and Eq. \ref{Eqn: Qat}). 



 We evaluate the performance of Skill-Critic on the robotic manipulation task  in Fig. \ref{fig:fetchresults}. As originally shown in the original paper \cite{rana2023residual}, ReSkill quickly learns a policy to clean the table, and outperforms other hierarchical methods like Hierarchical Actor Critic (HAC) \cite{levy2018learning} and PARROT \cite{singh2020parrot}, which are unable to learn anything meaningful on the task (see results in \cite{rana2023residual}). The alternative skill-embedding space in ReSkill speeds up exploration by biasing the HL policy towards skills relevant to the state. However, the LL residual policy in ReSkill only improves its value through the single-step reward $r(s,a)$. Skill-Critic can achieve an even higher reward by completing the task even \textit{faster}. We attribute this to the inter-related Q-function update that estimates the LL Q-function using the $H$-step reward estimate \textit{upon arrival} to a skill. The sparse reward can propagate further into the LL policy update, resulting in higher rewards. An interesting area for future research would be to apply ReSkill's alternative skill embedding to Skill-Critic.  However, we believe Skill-Critic's LL policy update is crucial to converge to the highest reward.

\subsection{Ablation Study}
\begin{figure}[b]
\centering

        \includegraphics[width=.25\textwidth,trim={0 0 19cm 1.2cm},clip]{figures/Qa_ablation.pdf}
    \includegraphics[width=.40\textwidth,trim={12cm 0 0 0},clip]{figures/Qa_ablation.pdf}
    \caption{Comparison of \textbf{independent} update of $Q^a_{\beta(s_{t+1})=1}$ from current $Q^a$ estimate and \textbf{Skill-Critic} update of $Q^a_{\beta(s_{t+1})=1}$ from current $Q^z$ estimate. HL policies are warm-started by SPiRL for 1 million steps, then trained for 1 million steps via Algorithm \ref{Alg:skill-critic-summary}. 
    \textbf{Top:} episode rewards during Algorithm \ref{Alg:skill-critic-summary} training. \textbf{Bottom:} State distribution of trajectories at convergence}
    \vspace{-2mm}
    \label{Fig: Qa_ablation}
\end{figure}



Skill-Critic uses the value \textit{upon arrival} to a new skill to estimate $Q_a$ by using $Q_{\bar{\phi}_z}$(Line 4 of Algorithm \ref{Alg:low-level}). 
Namely, when $\beta(s_{t+1})=0$, $Q^a$ is estimated with single-step discounting \eqref{Eqn: Qatau}, but when $\beta(s_{t+1})=1$, $Q^a$  is estimated with $H$-step discounting \eqref{Eqn: Qat}.
We perform an ablation study to test how this compares to the ``independent'' estimation of $Q^a$ and $Q^z$ in Fig. \ref{Fig: Qa_ablation}. \textbf{Independent} refers to estimating $Q^a$ only using Eq. \eqref{Eqn: Qatau} regardless of the value of $\beta(s_{t+1})$. \textbf{Skill-Critic} refers to the $Q^a$ estimate described in Algorithm \ref{Alg:low-level}. 
The ablation is performed in \textit{Curvy Tunnel}, and the high-MDP policy, $\pi_z$, and critic, $Q^z$, are warm-started for 1M steps of SPiRL. Fig. \ref{Fig: Qa_ablation} shows the episode rewards when $\pi_a$ and $\pi_z$ are trained (Algorithm \ref{Alg:skill-critic-summary}) for an additional 1M steps. 


The results indicate that the \textbf{independent} LL Q-value hinders exploration, and eventually, the policy can no longer find the goals. We hypothesize the distant goal's reward signal is too weak to guide the policy at states early in the rollout due to the single-step exponential discounting in Eq. \eqref{Eqn: Qatau}.
\textbf{Skill-Critic} includes $Q^z$ in the estimate of $Q^a$, which has two effects: 1) the $H$-step discounting of $Q^z$ is less prone to losing the sparse reward signal at earlier states in the rollout, and 2) the LL policy update employs state-skill values assigned by the HL policy. Thus, Skill-Critic outperforms independent Q-function estimation to consistently reach the goals.
% $^1$\footnote{$^1$To further comment on point 2: we have formulated $M^\mathcal{H}$ and $M^\mathcal{L}$ as two separate, parallel optimization problems. In theory, separate samples and convergence should be acquired before changing between the HL and LL problems, but Skill-Critic uses the same samples and single steps on each optimization problem, following the precedent in options frameworks \cite{zhang2019dac}. Intuitively, including $Q^z$ in the update of $Q^a$ may better link the parallel optimization problems, although future work is needed to show the exact mechanism and effect of this link.}
% Due to this desirable performance, we employ the \textbf{Skill-Critic} update for the rest of the experiments in this paper.

% In contrast, the 
% \textbf{Skill-Critic} LL Q-function update uses When $\beta(s_{t+1})=0$, estimation of $Q^a$ still relies on single-step discounting for LL policy refinement. However, when $\beta(s_{t+1})=1$, the current skill, $z_t$, is finished and a new one will be selected in the next time step. Here, when $\beta(s_{t+1})=1$, Skill-Critic employs Eqn. \eqref{Eqn: Qat} to estimate the current value of the skill. 

% The results suggest that the independent LL Q-value hampers exploration, leading to a rapid decline in episode returns, possibly because the distant goal's reward signal is too weak for earlier state guidance due to exponential discounting. In contrast, the Skill-Critic LL Q-value, incorporating $Q^z$ value, maintains exploration and rewards improvement without losing goal-finding ability. When $\beta(s_{t+1})=0$, $Q^a$ relies on single-step discounting, but with $\beta(s_{t+1})=1$, Skill-Critic employs Eqn. \eqref{Eqn: Qat} to estimate skill value. This benefits by 1) applying $H$-step discounting for HL Q-value ($Q^z$), capturing longer-horizon rewards better, and 2) informing the LL policy update with state-skill values from the HL policy. Due to these advantages, we exclusively use the Skill-Critic update for the remaining experiments in this paper.

==> submit1/submittedRAL/intro_related.tex <==
% ============ intro =============
\section{Introduction} \label{Sec:Intro}

Reinforcement learning (RL) has demonstrated remarkable success in various domains~\cite{mnih2015human,  wurman2022outracing}. %zhang2023learning,
However, standard RL algorithms often lack the ability to incorporate prior structure, knowledge, or experience, which may be necessary for complex tasks~\cite{li2022hierarchical, pertsch2021accelerating, pertsch2021guided, singi2023decision}. Incorporating prior experience by learning from demonstrations can facilitate efficient exploration~\cite{argall2009survey}. For example, statistical methods can infer the hidden structure of offline data and inform the decision-making process~\cite{pertsch2021accelerating, pertsch2021guided}. However, offline data alone may not suffice for determining an optimal policy, particularly when the data originates from simpler environments or pertains to intricate or stochastic tasks. In such cases, online policy optimization (referred to as \textit{fine-tuning}) is required to refine suboptimal policies \cite{nair2020awac,  nakamoto2023cal}. We present a hierarchical RL framework that leverages offline data to accelerate RL training without limiting its performance by the quality of offline data. 



\begin{figure}
\centering
\includegraphics[width=0.3\textwidth, trim={0 2pt 0 3pt},clip]{figures/overview_new.pdf}
\caption{Skill-Critic leverages low-coverage demonstrations to facilitate hierarchical reinforcement learning by (1) acquiring a basic skill-set from demonstrations that (2) guides online skill selection and skill improvement.}
\end{figure}

Our framework employs \textit{skills}, temporally extended sequences of primitive actions~\cite{kingma2013auto}. Previous works extract skills from unstructured data and transfer them to downstream RL tasks with a skill selection policy whose action space is the skill itself~\cite{sharma2019dynamics}. Skill-Prior RL (SPiRL)~\cite{pertsch2021accelerating} found learning a set of skills may not be adequate to guide skill selection; rather, exploration is improved when high-level skill selection is regularized by a data-informed prior distribution known as the skill prior. The skill prior informs high-level policy selection, but the low-level policy, i.e. the skill, is \emph{stationary}. However, when offline data is low-coverage or low-quality, stationary low-level skills may not suffice in complex downstream tasks. 

Our \emph{Skill-Critic} approach aims to leverage parallel high-level and low-level policy optimization to refine the skills themselves during skill selection. Intuitively, agents can use their experience to \textit{improve} their skill set, rather than being constrained to select skills from a stationary, offline library. 
We show this problem can be formulated as the parallel optimization of a high-level (HL) policy to select a skill and a low-level (LL) policy to select an action. We guide HL skill selection with a data-informed skill prior~\cite{pertsch2021accelerating}, and we extend this notion to initialize and regularize the LL skills using an action prior informed by offline data. Skill-Critic is reminiscent of discrete \textit{options}~\cite{zhang2019dac}; however, the offline data-informed, continuous skill space adds a unique structure for guiding and stabilizing the parallel policy optimization.


Our contributions are: (1) We formulate parallel optimization of the HL and LL policies to simultaneously select skills and improve the skill set, (2) We use an action prior to guide LL policy fine-tuning to improve the offline data-driven skill set, and (3) Our method \textit{improves} the skill set and performance in simulated navigation and robotic manipulation tasks and solves a new, sparse reward autonomous racing task in the complex Gran Turismo Sport environment.



% ========== related works =========
\section{Related Works} \label{Sec:RelatedWorks}

% \subsubsection{Offline RL}
% Offline RL algorithms use pre-collected demonstrations to learn optimal policies without environment interaction~\cite{levine2020offline}. When environment interaction is limited, offline RL can warm-start and accelerate online RL training~\cite{nair2020awac, singh2020cog, nakamoto2023cal}, which is referred to as \textit{fine-tuning}. However, the quality of offline priors highly relies on demonstrations. 
% RL fine-tuning performance can deteriorate when attempting to \textit{transfer} prior experience from one task to another~\cite{levine2020offline}. 

\subsubsection{Skill-transfer RL} 
Skill-transfer RL reuses pre-trained skills, i.e. sequences of actions, to accelerate RL training for downstream tasks~\cite{pertsch2021accelerating,pertsch2021guided, eysenbach2018diversity, hausman2018learning}. One commonly used approach is to learn a skill latent space from offline data using variational autoencoder (VAE)~\cite{kingma2013auto}. Then in downstream RL, an HL skill-selection policy is trained to select the optimal skill from the learned skill space. Thus, RL only needs to explore how to stitch temporally-extended action sequences, instead of searching for the optimal action at every time step. 
Extensions have learned priors for the HL policy from VAE training to guide and further accelerate RL training \cite{pertsch2021accelerating} and learned these skill priors from multiple datasets \cite{xu2022aspire}.
However, prior works often consider a \emph{stationary} skill space, constraining  performance to skills learned from offline data. 
% Adaptive Skill-Prior RL (ASPiRe)~\cite{xu2022aspire} alleviates this issue by enabling the RL agent to compose skill priors learned from multiple datasets, but LL policies are still stationary. 
% Nevertheless, the LL policies are still stationary, and the RL agent may still fail when the downstream task requires skills unseen in any available datasets.
% It motivates us to propose Skill-Critic, which is a hierarchical RL method that can effectively leverage low-coverage 
% or low-quality data for skill-transfer RL. 
\begin{figure*}[t]
    \centering
    \includegraphics[width = 0.715\textwidth]{figures/framework_cat_new.pdf}
    \caption{Hierarchical RL from a demonstration-guided latent space. \textbf{Left:} Offline data informs the skill embedding model with skill encoder (\textcolor{framework_yellow}{\textbf{yellow}}), skill prior (\textcolor{framework_green}{\textbf{green}}), and skill decoder (\textcolor{framework_blue}{\textbf{blue}}). Hyperparameter $\sigma_{\hat{a}}$ is augmented to the decoder to define the action prior. \textbf{Right:} HL (\textcolor{framework_red}{\textbf{red}}) and LL (\textcolor{framework_violet}{\textbf{purple}}) policies are fine-tuned on downstream tasks via our Skill-Critic algorithm. During fine-tuning, the HL and LL policies are regularized with the skill and action priors. }
    \label{fig:framework}
\end{figure*}


\subsubsection{Hierarchical RL} 
Hierarchical RL (HRL) decomposes long-horizon tasks into simpler sub-tasks, encouraging meaningful exploration during training~\cite{pateria2021hierarchical}. Commonly, algorithms employ intermediate variables, such as goals, options, or skills, to define subdomains that bridge high and low levels. Options HRL \cite{bacon2017option, zhang2019dac, li2020soac} uses discrete options that may not be sufficiently descriptive for complex tasks. Goal-conditioned HRL \cite{andrychowicz2017hindsight, eysenbach2022contrastive, nasiriany2019planning, pateria2021end, chane2021goal}  leverages automatic goal sampling methods (e.g. from prior experience or demonstrations) to train policies conditioned on goal states; however, the goal must be available from the state space.
In Skill-transfer RL \cite{eysenbach2018diversity, hausman2018learning}, the hierarchical policies could use a data-informed, continuous latent space, potentially representing a wider range of behaviors. Recent works use residual policies to augment a LL data-driven skill decoder  \cite{rana2023residual, won2022physics}. Skill-Critic provides an alternate mechanism for parallel HL and LL policy optimization: the decoder is an \textit{action prior} to guide the LL policy, and the skill prior guides the HL policy.
% Parallel policy training can alleviate this issue, but may be unstable or more sample intensive than single-layer RL because the agent must explore both the intermediate space and action space~\cite{bacon2017option}.


% Goal-conditioning hierarchical RL \cite{gupta2019relay, li2022hierarchical} requires additional methods for automatically sampling goals, such as hindsight relabeling \cite{andrychowicz2017hindsight, levy2018learning} to label experiences using future outcomes. 

%Single-layer hierarchical RL (such as skill-transfer RL) may fail to adequately adjust to the downstream environment.
% Recent advances in goal-conditioned hierarchical learning 
% Parallel policy learning can be accelerated by pre-trained goal-conditioned 
% policies from demonstrations~\cite{gupta2019relay, li2022hierarchical, levy2018learning} that require structured goal states to be defined. Conversely, we leverage \textit{skills}, thereby adding structure and prior experience to guide the parallel policy optimization problem. 




==> submit2/sections/abstract.tex <==
\begin{abstract}
Hierarchical reinforcement learning (RL) can accelerate long-horizon decision-making by temporally abstracting a policy into multiple levels. 
Promising results in sparse reward environments have been seen with \textit{skills}, i.e. sequences of primitive actions. Typically, a skill latent space and policy are discovered from offline data. However, the resulting low-level policy can be unreliable due to low-coverage demonstrations or distribution shifts.
As a solution, we propose the \emph{Skill-Critic} algorithm to fine-tune the low-level policy in conjunction with high-level skill selection. Our Skill-Critic algorithm optimizes both the low-level and high-level policies; these policies are initialized and regularized by the latent space learned from offline demonstrations to guide the parallel policy optimization. We validate Skill-Critic in multiple sparse-reward RL environments, including a new sparse-reward autonomous racing task in Gran Turismo Sport. The experiments show that Skill-Critic's low-level policy fine-tuning and demonstration-guided regularization are essential for good performance. Code and videos are available at our website: \href{https://sites.google.com/view/skill-critic}{https://sites.google.com/view/skill-critic}. 
\end{abstract}

\begin{IEEEkeywords}
Reinforcement Learning, Representation Learning, Transfer Learning
\end{IEEEkeywords}

==> submit2/sections/approach.tex <==

 \begin{figure*}[t]
    \centering
    \includegraphics[width = 0.715\textwidth]{figures/framework_cat_new.pdf}
    \caption{Hierarchical RL from a demonstration-guided latent space. \textbf{Left:} Offline data informs the skill embedding model with skill encoder (\textcolor{framework_yellow}{\textbf{yellow}}), skill prior (\textcolor{framework_green}{\textbf{green}}), and skill decoder (\textcolor{framework_blue}{\textbf{blue}}). Hyperparameter $\sigma_{\hat{a}}$ is augmented to the decoder to define the action prior. \textbf{Right:} HL (\textcolor{framework_red}{\textbf{red}}) and LL (\textcolor{framework_violet}{\textbf{purple}}) policies are fine-tuned on downstream tasks via our Skill-Critic algorithm. During fine-tuning, the HL and LL policies are regularized with the skill and action priors. }
    \label{fig:framework}
\end{figure*}
% =============== approach ==============
\section{Approach} \label{Sec:Approach}
We employ demonstration-informed, temporally abstracted skills in hierarchical RL to facilitate learning complex long-horizon tasks~\cite{pertsch2021accelerating}. The hierarchical policy consists of 1) a high-level (HL) policy, $\pi_z(z_t|s_t)$, that selects the best skill, $z_t$, given the current state, $s_t$; and 2) a low-level (LL) policy, $\pi_a(a_t|s_t,z_t)$, that selects the optimal action, $a_t$, given the state and selected skill. The HL policy selects skills from a learned continuous skill set $\mathcal{Z}$, i.e., $z_t\in\mathcal{Z}$. As in SPiRL~\cite{pertsch2021accelerating}, we consider a task in which we can extract an initial skill set from offline demonstrations to accelerate downstream RL training. We further consider cases where the extracted skill set is \emph{insufficient} for the downstream tasks, motivating our \textit{Skill-Critic} framework in Figure~\ref{fig:framework}.  In Stage 1, we leverage demonstrations to learn a skill decoder and skill prior that can accelerate RL training. In Stage 2, we leverage hierarchical RL to fine-tune \emph{both} the HL and LL policies, thus further improving the inadequate offline-learned skill set.



%comment
\subsection{Offline Skill Prior and Embedding Pre-Training (Stage 1)}\label{Sec:skillprior}
We assume access to demonstrations consisting of trajectories $\mathcal{D}=(\tau_0, \tau_1, ..., \tau_N)$, which each include states and actions at each time step $\tau=(s_t, a_t, ...)$. The demonstrations may not contain complete solutions for the downstream task; however, there are skills that can be transferred from the offline data by training an HL policy to select the best skills for a new task. Furthermore, the demonstrations include only a subset of potential skills or suboptimal skills, motivating the improvement of skills with RL fine-tuning of the LL policy.

We directly follow SkilD \cite{pertsch2021guided}, to embed a sequence of $H$ consecutive actions $a_{0:H-1}$, known as a \textit{skill},  into a latent space using a variational autoencoder (VAE) \cite{kingma2013auto}. The VAE objective contains three parts: 1) a reconstruction loss to minimize the difference between demonstration actions $a_k$ and those predicted by the decoder $\hat{a}_k = g_{\psi_a}(a|s,z)$; 2) regularization on the encoder $q_\zeta(z|s_{0:H-1},a_{0:H-1})$ to align the latent distribution with a standard normal distribution; and 3) a KL-divergence term to train the skill prior $p_{\psi_z}(z|s_0)$ to match the posterior distribution inferred from the encoder. The first two terms are standard components of a VAE \cite{kingma2013auto}, and the third term trains the skill prior that can accelerate downstream RL \cite{pertsch2021accelerating}. We use a state-dependent decoder, $g_{\psi_a}(a|s,z)$ \cite{pertsch2021guided}, and augment the state with a one-hot vector corresponding to the time since skill selection for a more informative policy.

The skill prior parameterizes a Gaussian distribution and can be used directly to initialize and regularize a downstream HL policy \cite{pertsch2021accelerating, pertsch2021guided}.
In the next section, we extend this notion to an \textit{action prior} that can initialize and regularize a downstream LL policy.
The pre-trained (deterministic) skill decoder is an obvious choice, as previous works directly use the decoder as the LL policy  \cite{pertsch2021accelerating, pertsch2021guided}. Thus, we define a Gaussian action prior, denoted as $p_{\bar{\psi}_a}(a|z,s)=\mathcal{N}(\mu_{\hat{a}}, \sigma_{\hat{a}})$, with mean given by the skill decoder: $\mu_{\hat{a}}= g_{\psi_a}$. While the variance, $\sigma_{\hat{a}}$, is a hyperparameter, this action prior provides a more informative prior than SAC's entropy (unit Gaussian prior)\cite{pertsch2021accelerating}.  


\subsection{Hierarchical Skill-Prior and Action-Prior Regularized RL Fine-tuning (Stage 2)}\label{Sec:HRLregularize}
% \begin{comment}

\begin{algorithm}[b]
\small
\caption{The Skill-Critic RL Algorithm} \label{Alg:skill-critic-summary}
\begin{algorithmic}[1]
% \renewcommand{\arraystretch}{2.0}
\STATE \textbf{Inputs:} Skill prior $p_{\psi_z}(z|s)$ and action prior $p_{\bar{\psi}_a}(a|s,z)$
%, initial network weights, hyperparameters
\FOR{each iteration $i = 0, 1, 2, ...$}
\FOR{each environment step}
\IF{$t \mod H == 0$}
\STATE Sample skill $z\sim \pi_{\theta_z}(\cdot|s)$
\ENDIF
\STATE Sample action $a_t\sim \pi_{\theta_a}(\cdot|s_t,z)$
\STATE Perform action; add  $\{s,z,a,r,s'\}_t$ to replay buffer
\ENDFOR
\FOR{$t = 0,H, 2H,...$ and $t^*\doteq t+H$ }
\STATE Update HL policy, critic, and temperature towards Eqn.~\eqref{Eqn:HL obj} (i.e SPiRL \cite{pertsch2021accelerating})
\ENDFOR
\FOR{$t = 0,1,2,...$ and $t'\doteq t+1$}
\STATE Update LL policy, critic, and temperature towards Eqn.~\eqref{Eqn:LL obj} via Algorithm~\ref{Alg:low-level} \textbf{if} $i\geq N_{\textrm{HL-warm-up}}$
\ENDFOR
\ENDFOR

\STATE \textbf{Return} trained HL policy $\pi_{\theta_z}$ and 
 LL policy $\pi_{\theta_a}$

\end{algorithmic}
\end{algorithm}
% \end{comment}

We present Skill-Critic (Alg. \ref{Alg:skill-critic-summary}), 
which uses a parallel MDP structure to optimize the HL and LL policy with guidance from the pre-trained skill prior and action prior. To derive the parallel optimization of $\pi_a$ and $\pi_z$, we first note that the learned skill space forms a semi-MDP endowed with skills in Section \ref{subsub:semiMDP}. This semi-MDP formulation can be written as a parallel MDP formulation (Section \ref{subsub:parallel}), so that we optimize the HL policy $\pi_{z}$ on a ``high-MDP'' $M^\mathcal{H}$ and the LL policy $\pi_{a}$ on a ``low-MDP'' $M^\mathcal{L}$. Finally, in Sections \ref{subsub:high} and \ref{subsub:low}, the HL and LL policy optimizations are guided by the pre-trained skill prior, $p_{\psi_z}(z|s)$, and action prior, $p_{\bar{\psi}_a}(a|s,z)$.  In each policy optimization, we initialize the trained policy with the corresponding pre-trained prior policy and augment the objective function with the KL divergence between the trained policy and its prior. To stabilize hierarchical training, we train the HL policy for $ N_{\textrm{HL-warm-up}}$ steps prior to training the LL policy.

 Our formulation makes three notable improvements on prior works: 1.) we employ a \textit{skill-based} parallel MDP formulation to update the HL and LL policies in parallel, 2.) we introduce a LL Q-function estimate using known relationships between state-action values on the MDPs to stabilize optimization, and 3.) we extend soft actor-critic (SAC)~\cite{haarnoja2018soft} with non-uniform priors \cite{pertsch2021accelerating} to guide the LL policy update with the action prior.


\subsubsection{Semi-MDP endowed with skills}
\label{subsub:semiMDP}The hierarchical policies $\pi_a$ and $\pi_z$ form an MDP endowed with skills. We argue this is a semi-MDP similar to the one defined in the options framework \cite{sutton1999between}, as skills are continuous, fixed-duration options.
 The state space $\mathcal{S}$ consists of the environment states that are augmented with a one-hot encoding of the time index since the beginning of the active skill, $k_t \doteq (t \mod H )\in \mathcal{K}\doteq\{0,1,...H-1\}$. Following options notation \cite{zhang2019dac}, the skill is a triple $(\mathcal{I}, \pi_a, \beta)$, with initiation set $\mathcal{I}$, intra-skill policy $\pi_a:\mathcal{S}\times \mathcal{Z}\rightarrow \mathcal{A}$, and termination function $\beta: \mathcal{S}\rightarrow [0,1]$. We set $\mathcal{I}$ to the subset of states in $\mathcal{S}$ where $k=0$, meaning skills are only initiated after a fixed horizon $H$ since the previous skill was initiated. The termination function is  $\beta(s_t)\doteq\beta_t\doteq \mathbb{I}_{k_t=0}$, which takes value $\beta_t=1$ when $k_t=0$ and $\beta_t=0$ otherwise. The semi-MDP consists of states, actions, skills,  reward, transition probability, initial state distribution, and discount factor as listed in Table \ref{tab:mdp}.
 
% The semi-MDP consists of $M^\Omega \doteq \{\mathcal{S}, \mathcal{A}, \mathcal{Z}, R, p, p_0, \gamma\}$, of states, actions, skills,  reward, transition probability, initial state distribution, and
% discount factor.  The RL objective, $\mathbb{E}_{\pi_a,\pi_z,\beta}[\Sigma_{t=0}^{T-1} \gamma^t r_t]$, maximizes the expected discounted rewards induced by $\pi_a$, $\pi_z$, and $\beta$.

To solve the RL objective, we adapt the value functions from option-critic~\cite{bacon2017option} to continuous, fixed horizon skills:
\begin{equation}\label{eq:semiMDP}\begin{gathered}
V^\Omega_z\left( s_{t + 1} \right) = \mathbb{E}_{z_{t + 1}\sim\pi_{\theta_{z}}}\left\lbrack {Q_z^{\Omega}\left( {s_{t + 1},z_{t + 1}} \right) } \right\rbrack\\
Q^{\Omega}_z\left( {s_{t},z_{t}} \right) = \mathbb{E}_{a_{t}\sim\pi_{\theta_{a}}}\left\lbrack {Q^{\Omega}_a\left( {s_{t},z_{t},a_{t}} \right) } \right\rbrack\\
Q^{\Omega}_a\left( {s_{t},z_{t},a_{t}} \right) = r\left( {s_{t},a_{t}} \right) + \gamma\mathbb{E}_{a_{t + 1}\sim\pi_{\theta_{a}},\pi_{\theta_{z}}}\left\lbrack {U\left( {z_{t},s_{t + 1}} \right)} \right\rbrack\\
U\left( {z_{t},s_{t + 1}} \right) = \left\lbrack {1 - \beta_{t + 1}} \right\rbrack Q^{\Omega}_z\left( {s_{t + 1},z_{t}} \right) +\beta_{t + 1} V^{\Omega}_z\left( s_{t + 1} \right).
\end{gathered}
\end{equation}
Here $V^\Omega_z$ is the value of the state $s_t$, $Q_z^\Omega$ is the value of selecting skill $z_t$ from $s_t$, and $Q^\Omega_a$ is the value of selecting action $a_t$ from state $s_t$ and skill $z_t$.
Simplifying for fixed horizon skills, when $\beta(s_{t+1})=0$ during rollout of a skill,
\begin{equation}\label{Eqn: Qa_noreg_b0}
\begin{gathered}
    Q^\Omega_{a, \beta_{t+1}=0} = r(s_t,a)+\mathbb{E}_{\pi_a,\pi_z}[Q^\Omega_a(s_{t+1},z_{t+1},a_{t+1})].
    \end{gathered}
\end{equation}
and when $\beta(s_{t+1})=1$ at selection of the next skill
\begin{equation}\label{Eqn: Qa_noreg_b1}
            Q^\Omega_{a, \beta_{t+1}=1} = r(s_t,a)+\mathbb{E}_{\pi_a,\pi_z}[Q^\Omega_z(s_{t+1},z_{t+1})].
\end{equation}




\subsubsection{Formulation as two augmented MDPs} \label{subsub:parallel}

The semi-MDP requires special algorithms~\cite{bacon2017option}, which are difficult to augment with skill and action prior regularization. 
Rather, we re-formulate the semi-MDP as two parallel augmented MDPs by adapting an options-based parallel MDP framework, Double Actor Critic (DAC) \cite{zhang2019dac}, to our continuous, fixed-horizon skills. Thus, standard RL algorithms can be used to learn each policy \cite{zhang2019dac}. 
In Table \ref{tab:mdp}, we derive the formulation with a similar notation to DAC (Section 3) by  replacing discrete options, $O\sim \mathcal{O}$, with skills, $Z\sim \mathcal{Z}$. The HL policy $\pi_z$ selects skills in the high-MDP $M^\mathcal{H}$, and the LL policy $\pi_a$ selects actions in the low-MDP $M^\mathcal{L}.$

 To form the high-MDP $M^\mathcal{H}$, the state is composed of the current state and skill $\textbf{s}_{t}^\mathcal{H}\doteq (z_{t-1}, s_t)$, and the action is the next skill $\textbf{a}_t^\mathcal{H}\doteq z_t$. We define $p_z$ as the transition probability function from the current state and skill to the next state:
\begin{equation}\label{eq:skill_transition_function}
    p_z\left(s_{t+1} | s_t, z_t\right)\doteq \mathbb{E}_{ a\sim \pi_{a}\left(a | s_t, z_t\right)} \left[p\left(s_{t+1} | s_t, a\right)\right].
\end{equation}
Eq. \ref{eq:skill_transition_function} is analogous to the first equation in Section 2 of DAC; however, we define $p_z$ by taking the expectation over actions instead of using a discrete probabilistic estimate.  The transition probability, $p^\mathcal{H}$,  on $M^{\mathcal{H}}$ is defined with $p_z$ in Table \ref{tab:mdp},
 where $\mathbb{I}$ is the indicator function. In the initial distribution $p_0^\mathcal{H}$, it is not necessary to define a dummy skill \cite{zhang2019dac}, since we always start with skill selection from $\pi_z(z_t|s_t)$ at $t=0$. 

Since $\pi^\mathcal{H}$ executes a skill for $H$ time steps, at which point $\pi_{\theta_z}$ selects a new skill, we define an $H$-step reward: 
\begin{equation}\label{eq:hstepreward}
    \tilde{r}_H\left(s_t, z_t\right)\doteq \mathbb{E}_{ a_t\sim \pi_{a}\left(a \mid s_t, z_t\right)} \left[\Sigma_{\tau = t}^{t+H-1} r(s_\tau, a_\tau)\right],
\end{equation} 
where $\tilde{r}_H(s_t,z_t)$ is the sum of rewards when executing $z_t$ from $s_t$ for $H$ steps. The corresponding RL objective on  $M^\mathcal{H}$ (Table 1) maximizes the sum of $H$-step rewards $\tilde{r}_H$ with discount factor $\gamma_z$, which is valid when $\tilde{r}_H$ is evaluated only at instances when skills change ($\beta(s)=1$) \cite{pertsch2021accelerating}. This formulation is a slight deviation from DAC's single-step reward, but it improves performance on long-horizon tasks~\cite{pertsch2021accelerating}. 

% To emphasize the environment reward is discounted every $H$ steps on $M^\mathcal{H}$, we denote the discount factor for the HL objective in Table \ref{tab:mdp} as $\gamma_z$. 

% Further, the RL objective is still valid on $M^\mathcal{H}$, since  $r^\mathcal{H}\doteq \tilde{r}_H$ when evaluated only at instances when skills change ($\beta(s)=1$) \cite{pertsch2021accelerating}. 



% \begin{equation}
%     r_z\left(s_t, z_t\right)\doteq \mathbb{E}_{ a_t\sim \pi_{a}\left(a \mid s_t, z_t\right)} \left[r\left(s_t,  a_t\right)\right].
% \end{equation}
 
%  Thus, we can write $M^{\mathcal{H}}$ as a regular MDP:
% \begin{equation}
%         \begin{aligned}
%         & 
%         \mathcal{S}^{\mathcal{H}} \doteq  \mathcal{Z}\times\mathcal{S}, \quad \mathcal{A}^{\mathcal{H}} \doteq \mathcal{Z} \\ 
% M^{\mathcal{H}} & \doteq\left\{\mathcal{S}^{\mathcal{H}}, \mathcal{A}^{\mathcal{H}}, p^{\mathcal{H}}, p_0^{\mathcal{H}}, r^{\mathcal{H}}, \gamma\right\},  \\
% p^{\mathcal{H}}\left(S_{t+1}^{\mathcal{H}} \mid S_t^{\mathcal{H}}, A_t^{\mathcal{H}}\right) & \left. \doteq p^{\mathcal{H}}\left( (z_t,s_{t+1}) \mid (z_{t-1},s_t), A_t^{\mathcal{H}}\right)\right) \\ & \doteq \mathbb{I}_{A_t^{\mathcal{H}}=z_t} p_z\left(s_{t+1
% } \mid s_t, z_t\right) \\ 
% p_0^{\mathcal{H}}\left(S_0^{\mathcal{H}}\right) & \doteq p_0^{\mathcal{H}}\left((z_{-1},s_0)\right)  \doteq p_0\left(s_0\right), \\ 
% r^{\mathcal{H}}\left(S_t^{\mathcal{H}}, A_t^{\mathcal{H}}\right) & \doteq r^{\mathcal{H}}\left((z_{t-1}, s_t), z_t\right) \doteq r_z\left(s_t, z_t\right), 
% \end{aligned}
% \end{equation}


We define the Markov policy $\pi^\mathcal{H}$ on $M^\mathcal{H}$ as 
\begin{equation}\label{Eqn: pi_H}
\begin{aligned}
    \pi^{\mathcal{H}}\left(\textbf{a}_t^{\mathcal{H}} \mid \textbf{s}_t^{\mathcal{H}}\right) & \doteq \pi^{\mathcal{H}}\left(z_t \mid (z_{t-1}, s_t)\right) \\ \doteq (1&-\beta(s_t)) \mathbb{I}_{z_{t-1}=z_t} + \beta(s_t)\pi_z \left(z_t \mid s_t\right).
    \end{aligned}
\end{equation}
Eq.~\eqref{Eqn: pi_H}  shows that the previous skill is used until  $\beta(s_t)=1$; then a new skill is selected via $\pi_z$. 
Unlike DAC, we use  $\beta$'s definition to simplify \eqref{Eqn: pi_H} to only be a function of $\pi_z$ and $\beta$.




\begin{table*}[]
\setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.35}
    \centering

        \caption{MDP Formulations for solving skill-based HRL}
    \label{tab:mdp}
    \begin{tabular}{|c|c|c|c|}
    \hline 
        & \textbf{Original semi-MDP}, $M^{\Omega}$& \textbf{High-MDP}, $M^\mathcal{H}$ & \textbf{Low-MDP}, $M^\mathcal{L}$\\
        %%%%%%%%%%
        \hline
        \textbf{MDP Tuple} & $M^\Omega \doteq \{\mathcal{S}, \mathcal{A}, \mathcal{Z}, p, p_0, r, \gamma\}$ & $M^{\mathcal{H}} \doteq\left\{\mathcal{S}^{\mathcal{H}}, \mathcal{A}^{\mathcal{H}}, p^{\mathcal{H}}, p_0^{\mathcal{H}}, r^{\mathcal{H}}, \gamma_z\right\}$ & $M^{\mathcal{L}} \doteq\left\{\mathcal{S}^{\mathcal{L}},\mathcal{A}^{\mathcal{L}}, p^{\mathcal{L}}, p_0^{\mathcal{L}}, r^{\mathcal{L}}, \gamma\right\}$\\
        \hline         %%%%%%%%%%
        \textbf{State Space} & $s_t\in\mathcal{S}$ &$\textbf{s}^\mathcal{H}_t\doteq (z_{t-1},s_t)\in\mathcal{S}^{\mathcal{H}}$  & $\textbf{s}^\mathcal{L}_t\doteq (s_t, z_t)\in\mathcal{S}^{\mathcal{L}}$\\ \hline
       \textbf{ Action Space} & $a_t\in \mathcal{A}$& $\textbf{a}_t^\mathcal{H} \doteq z_t \in \mathcal{A}^\mathcal{H}$ &  $\textbf{a}_t^\mathcal{L} \doteq a_t \in \mathcal{A}^\mathcal{L}$\\ 
        \hline
        \textbf{Latent Space }& $z_t\in \mathcal{Z}$ & - & -\\
        \hline         %%%%%%%%%%
        \multirow{3}{*}{\begin{tabular}{c}\textbf{Transition}\\ \textbf{Probability}\end{tabular}} & \multirow{3}{*}{ $p(s_{t+1}|s_t, a_t)$}
        & \multicolumn{1}{l|}{$p^{\mathcal{H}}\left(\textbf{s}_{t+1}^{\mathcal{H}} \mid \textbf{s}_t^{\mathcal{H}}, \textbf{a}_t^{\mathcal{H}}\right)  $ }  & \multicolumn{1}{l|}{$p^{\mathcal{L}}\left(\textbf{s}_{t+1}^{\mathcal{L}} \mid \textbf{s}_t^{\mathcal{L}}, \textbf{a}_t^{\mathcal{L}}\right)$}\\ %%%%%%%%%%
& & \multicolumn{1}{l|}{$\doteq p^{\mathcal{H}}\left( (z_t,s_{t+1}) \mid (z_{t-1},s_t), a_t^{\mathcal{H}})\right)$} & \multicolumn{1}{l|}{ $ \doteq p^{\mathcal{L}}\left(\left(s_{t+1}, z_{t+1}\right) \mid\left(s_t, z_t\right), a_t\right)$}\\ %%%%%%%%%%
& & \multicolumn{1}{l|}{$\doteq \mathbb{I}_{\textbf{a}_t^{\mathcal{H}}=z_t} p_z\left(s_{t+1
} \mid s_t, z_t\right) $} & \multicolumn{1}{l|}{$\doteq p\left(s_{t+1} \mid s_t, a_t\right) p\left(z_{t+1} \mid s_{t+1}, z_t\right) $}\\ %%%%%%%%%%
\hline
\textbf{Init. Distribution }& $p_0(s_{0})$ & $p_0^{\mathcal{H}}(\textbf{s}_0^{\mathcal{H}})  \doteq p_0^{\mathcal{H}}((z_{-1},s_0))  \doteq p_0(s_0)$ & $p_0^{\mathcal{L}}(\textbf{s}_0^{\mathcal{L}}) \doteq p^{\mathcal{L}}((s_0, z_0))  \doteq  \pi_z(z_0|s_0)p_0(s_0)$ \\ %%%%%%%%%%
\hline 
\multirow{2}{*}{\textbf{Reward}} & \multirow{2}{*}{$r(s_t, a_t)$} & \multicolumn{1}{l|}{$r^{\mathcal{H}}(\textbf{s}_t^{\mathcal{H}}, \textbf{a}_t^{\mathcal{H}})\doteq r^{\mathcal{H}}((z_{t-1}, s_t), z_t)$}& \multicolumn{1}{c|}{$r^{\mathcal{L}}(\textbf{s}_t^{\mathcal{L}}, \textbf{a}_t^{\mathcal{L}})\doteq r^{\mathcal{L}}((s_t, z_t), a_t) $} \\%%%%%%%%%%
& & $\doteq \tilde{r}_H(s_t,z_t) $ &  $ \doteq r(s_t, a_t)$\\%%%%%%%%%%
\hline
\textbf{RL Objective} & $\mathbb{E}_{\pi_a,\pi_z}[\Sigma_{t=0}^{T-1} \gamma^t r_t]$, $\gamma=.99$ & $\mathbb{E}_{\pi_a,\pi_z}[\Sigma_{t=0}^{T-1} \gamma_z^t \tilde{r}_H(s_t, z_t)]$, $\gamma_z=.99$& $\mathbb{E}_{\pi_a,\pi_z}[\Sigma_{t=0}^{T-1} \gamma^t r(s_t,a_t)]$, $\gamma=.99$ \\
\hline
\multirow{3}{*}{\begin{tabular}{c}\textbf{Q \& Value}\\ \textbf{Functions}\end{tabular}} & $V_z^\Omega(s_{t+1})$: state value& $Q^\mathcal{H}(\textbf{s}_t^\mathcal{H}, \textbf{a}_t^\mathcal{H})\doteq Q^z(s_t,z_t)$&$Q^\mathcal{L}(\textbf{s}^\mathcal{L},\textbf{a}^\mathcal{L})\doteq Q^a(s,z,a)
$ \\
 & $Q_z^\Omega(s_t, z_t)$: value of $(s_t, z_t)$ & $V^{\mathcal{H}}(\textbf{s}_t^{\mathcal{H}})\doteq V^{\mathcal{H}}(s_t)$&$V^{\mathcal{L}}(\textbf{s}_t^{\mathcal{L}})\doteq V^{\mathcal{L}}((s_t, z_t))$\\
& $Q_a^\Omega(s_t, z_t, a_t)$: value of $a_t$ in $(s_t, z_t)$ & applied every $H$ steps& applied every $1$ step\\
\hline
    \end{tabular}
\end{table*}
In the low-MDP, $M^\mathcal{L}$, the state is composed of the current state and next skill, $\textbf{s}_{t}^\mathcal{L}\doteq (s_t, z_t)$, and the action is the action $\textbf{a}^\mathcal{L}\doteq a_t$. The transition probability, initial distribution, and reward directly follow using our definition of $\beta$ and DAC.
%  Then $M^{\mathcal{L}}$ is the regular MDP
% \begin{equation}
% \begin{aligned}
% \mathcal{S}^{\mathcal{L}} & \doteq \mathcal{S} \times \mathcal{Z}, \quad \mathcal{A}^{\mathcal{L}} \doteq \mathcal{A} \\ 
%     M^{\mathcal{L}} & \doteq\left\{\mathcal{S}^{\mathcal{L}}, \mathcal{A}^{\mathcal{L}}, p^{\mathcal{L}}, p_0^{\mathcal{L}}, r^{\mathcal{L}}, \gamma\right\} \\
% p^{\mathcal{L}}\left(S_{t+1}^{\mathcal{L}} \mid S_t^{\mathcal{L}}, A_t^{\mathcal{L}}\right) & \doteq p^{\mathcal{L}}\left(\left(s_{t+1}, z_{t+1}\right) \mid\left(s_t, z_t\right), a_t\right) \\ &\doteq p\left(s_{t+1} \mid s_t, a_t\right) p\left(z_{t+1} \mid s_{t+1}, z_t\right) \\
% p_0^{\mathcal{L}}\left(S_0^{\mathcal{L}}\right) & \doteq p^{\mathcal{L}}\left(\left(s_0, z_0\right)\right)  \doteq  \pi_z\left(z_0|s_0\right)p_0\left(s_0\right) \\ 
% r^{\mathcal{L}}\left(S_t^{\mathcal{L}}, A_t^{\mathcal{L}}\right) & \doteq r^{\mathcal{L}}\left(\left(s_t, z_t\right), a_t\right)  \doteq r\left(s_t, a_t\right).
% \end{aligned}
% \end{equation}
We define a Markov policy $\pi^\mathcal{L}$ on $M^\mathcal{L}$ as the LL policy $\pi_a$:
\begin{equation}
    \pi^{\mathcal{L}}\left(\textbf{a}_t^{\mathcal{L}} \mid \textbf{s}_t^{\mathcal{L}}\right) \doteq \pi^{\mathcal{L}}\left(a_t \mid\left(s_t, z_t\right)\right) \doteq \pi_{a}\left(a_t \mid s_t,z_t\right).
\end{equation}
It follows that when we fix  $\pi_a$ and optimize $\pi^\mathcal{H}$, we are optimizing $\pi_z$. Likewise, when we fix $\pi_z$ and optimize $\pi^\mathcal{L}$, we are optimizing $\pi_a$~\cite{zhang2019dac}. This implies that any policy optimization algorithm can be used to optimize $\pi^\mathcal{H}$ and $\pi^\mathcal{L}$.



% \clearpage
\subsubsection{High-MDP Policy Optimization} \label{subsub:high} To optimize $\pi^\mathcal{H}$ on $M^\mathcal{H}$, policy $\pi_{z}$ is parameterized by $\theta_z$ (denoted $\pi_{\theta_z}$), and we fix $\pi^\mathcal{L}$. The skill prior, $p_{\psi_z}$, is a prior distribution for $\pi_{\theta_z}$, and $\theta_z$ is initialized with $\psi_z$. 
The \textit{HL update} in Fig.~\ref{fig:framework} solves 
\begin{equation}
\label{Eqn:HL obj}
\begin{aligned}
\underset{\theta_z}{\operatorname{argmax}} \;\mathbb{E} _{\pi_{\theta_z},\pi^\mathcal{L}}&\left[\sum_{t=\{0, H, 2H, \hdots \}}^{\infty} \gamma_z^t \Big(\tilde{r}_H(s_t, z_t) \right. \\
& \left. -\alpha_z D_{K L}[\pi_{\theta_z}(z_t | s_t) \| p_{\psi_z}(z_t | s_t)]\Big)\right].
\end{aligned}
\end{equation}
where the regularization term is weighted with temperature $\alpha_z$.
We solve \eqref{Eqn:HL obj} using the Bellman operator on $M^\mathcal{H}$:
\begin{equation}\label{Eqn: spirl_bellman}
    \begin{aligned}
        &\mathcal{T}^{\pi_z} Q^\mathcal{H}\left(s_t, z_t\right)=\tilde{r}_H\left(s_t, z_t\right)+\gamma_z\mathbb{E}_{p^{\mathcal{H}}}\left[V^\mathcal{H}\left(s_{t+1}\right)\right]\\
         &V^\mathcal{H}\left(s_t\right)=\mathbb{E}_{z_t \sim \pi_z}\big[Q^\mathcal{H}\left(s_t, z_t\right) \\& \qquad \qquad \qquad-D_{\mathrm{KL}}\left[\pi_z\left(z_t | s_t\right) \| p_{\psi_z}\left(z_t |s_t\right)\right]\big].
    \end{aligned}
\end{equation}
The value function $V^\mathcal{H}$ and Q-function $Q^\mathcal{H}$ are defined on $M^\mathcal{H}$ using the Bellman operator in SPiRL \cite{pertsch2021accelerating}, which is proven to solve \eqref{Eqn:HL obj} by adapting SAC \cite{haarnoja2018soft}. 
The $H$-step reward, $\tilde{r}_H$, implies  $Q^\mathcal{H}(\textbf{s}^{\mathcal{H}}_t,\textbf{a}_t^{\mathcal{H}})\doteq Q^z(s_t,z_t)$, and the state-skill value estimation is discounted every $H$ steps, which can improve performance by increasing the effect of sparse rewards \cite{pertsch2021accelerating}.



\subsubsection{Low-MDP Policy Optimization}\label{subsub:low} To optimize $\pi^\mathcal{L}$ on $M^\mathcal{L}$, policy $\pi_{a}$ is parameterized by $\theta_a$ (denoted $\pi_{\theta_a}$), and we fix $\pi^\mathcal{H}$. The action prior learned from offline demonstrations, $p_{\bar{\psi}_a}$, is a prior distribution for $\pi_{\theta_a}$, and $\theta_a$ is initialized with $\bar{\psi}_a$. The regularized objective with temperature $\alpha_a$ is
\begin{equation} \label{Eqn:LL obj}
\begin{aligned}
\underset{\theta_a}{\operatorname{argmax}} \; &\mathbb{E}_{\pi_{\theta_a}, \pi^\mathcal{H}}\left[\sum_{t=0}^{\infty} \gamma^t \Big(r\left(s_t, a_t\right) \right. \\
& \left. -\alpha_a D_{K L}\left[\pi_{\theta_a} (a_{t} | s_{t}, z_t) \| p_{\bar{\psi}_a}(a_{t}  | s_{t}, z_t, )\right]\Big)\right],
\end{aligned}
\end{equation}
corresponding to the \bluetext{\textit{LL update}} in Fig.~\ref{fig:framework}.  Algorithm~\ref{Alg:low-level} updates the LL policy by adapting  KL-divergence regularized SAC to solve \eqref{Eqn:LL obj}. We define the Bellman operator on $M^\mathcal{L}$:
\begin{equation}\label{Eqn: ll_bellman}
    \begin{aligned}
       & \mathcal{T}^{\pi_a} Q^\mathcal{L}\left((s_t,z_t), a_t\right)=r\left(s_t, a_t\right)+\gamma \mathbb{E}_{p^\mathcal{L}}\left[V^\mathcal{L}\left((s_{t+1},z_{t+1})\right)\right]\\
        &V^\mathcal{L}\left((s_t,z_t)\right)=\mathbb{E}_{a_t \sim \pi_{a}}\big[Q^\mathcal{L}\left((s_t,z_t), a_t\right)\\ & \qquad \qquad -D_{\mathrm{KL}}\left[\pi_a\left(a_t | (s_t,z_t)\right) \| p_{\bar{\psi}_a}\left(a_t | (s_t,z_t)\right)\right]\big].
    \end{aligned}
\end{equation}
Similar to the HL update, the entropy regularization in SAC is replaced with the deviation of the policy $\pi_{\theta_a}$ from the prior $p_{\bar{\psi}_z}$. Dual gradient descent on the temperature $\alpha_a$ \cite{haarnoja2018soft, pertsch2021accelerating} ensures that the expected divergence between LL policy and
the action prior is equal to the chosen target divergence $\delta_a$ on Line 9. 
The LL Q-value,
$Q^a(s,z,a),
$ estimates the value of the state-skill pair and action with 1-step discounting  \eqref{Eqn:LL obj}.



When estimating $Q^a$ with \eqref{Eqn: ll_bellman}, far-horizon rewards have an exponentially diminishing effect. Practically,  this led to poor performance in sparse reward environments. 
Inspired by the relationship between Q-functions on the semi-MDP \eqref{eq:semiMDP}, we investigate if the longer-horizon HL Q-value can inform LL policy optimization of the value that the HL policy is assigning to state-skill pairs. Thus, sparse rewards propagate to earlier states. We observe in the semi-MDP that $V_z^\Omega$ is analogous to the value of skills, meaning $V_z^\Omega$ is analogous to the value function on the high-MDP, $V^\mathcal{H}$. Likewise, $Q^\Omega_z$ is analogous to the value of state-skill pairs, meaning $Q^\Omega_z$ is analogous to the value function on the low-MDP, $V^\mathcal{L}$. 



The semi-MDP \eqref{eq:semiMDP} does not include policy regularization. To incorporate our non-uniform prior into $Q^a$ estimation, we note that the regularization terms in \eqref{Eqn: spirl_bellman} and \eqref{Eqn: ll_bellman} appear in the definition of $V^\mathcal{H}$ and $V^\mathcal{L}$. 
We follow this precedent as we introduce regularization into \eqref{Eqn: Qa_noreg_b0}  and \eqref{Eqn: Qa_noreg_b1}.
We define
\begin{equation} \label{Eqn: Qat}
\begin{aligned}
Q^a_{\beta(s_{t+1})=1}\left(s_{t}, z_{t}, a_{t}\right)= & r\left(s_t, a_t\right)+\gamma \mathbb{E}_{\pi_z}\big[Q^z\left(s_{t+1}, z_{t+1}\right)\\
-\alpha_z D_{K L} & [\pi_{\theta_z}(z_t | s_t) \| p_{\psi_z}(z_t | s_t)] \big],
\end{aligned}
\end{equation}
 to  estimate $Q^a$ at the end of a skill (Line 4, Alg. \ref{Alg:low-level}) and
\begin{equation} \label{Eqn: Qatau}
\begin{aligned}
 Q^a \left(s_{t}, z_t, a_{t}\right)= & r(s_t,a_t)+\gamma \mathbb{E}_{\pi_a, \pi_z}\big[Q^a(s_{t+1},z_{t+1},a_{t+1}) \\
-\alpha_a D_{K L} & \left[\pi_{\theta_a} (a_{t} | s_{t}, z_t) \| p_{\bar{\psi}_a}(a_{t}  | s_{t}, z_t, )\right] \big], \\
\end{aligned}
\end{equation}
 otherwise. While the semi-MDP assumptions do not strictly hold for the regularized objective \eqref{Eqn:LL obj}, we find that using $Q^z$ to estimate $Q^a$ leads to faster, stable convergence. 



 \begin{algorithm}[t] 
\caption{Skill-Critic Low-MDP Update} \label{Alg:low-level}
\begin{algorithmic}[1]
% \renewcommand{\arraystretch}{2.0}
\STATE \textbf{Inputs: } Current iteration's HL parameters: $\bar{\phi}_z, \theta_z$; priors $p_z, p_\psi$, hyperparameters
\FOR{each $t = 0,1,2,...$ and $t'=t+1$ in buffer}
\IF{$k_{t}==H-1, \quad$ (where $k_{t}= t\mod H$)}
\STATE $\bar{Q}^{a} = Q^a_{\beta(s')=1}(s, z, a)$ using $Q_{\bar{\phi}_z}^z$ in \eqref{Eqn: Qat} \\ \COMMENT{Estimate LL Q-value  \textit{upon arrival} to new skill} \label{line:new_skill}
\ELSE
\STATE $\bar{Q}^{a} = Q^a_{\beta(s')=0}(s, z, a)$ using $Q_{\bar{\phi}_a}^z$ in \eqref{Eqn: Qatau} \\ \COMMENT{Estimate LL Q-value  within current skill}
\ENDIF
\STATE $\theta_{a}\leftarrow $ step on \eqref{Eqn:LL obj} using $Q_{\phi_a}^a$ \COMMENT{update LL policy parameters}
\STATE $\phi_{a} \leftarrow \phi_{a} - \lambda_{Q_a} \nabla_{\phi_{a}} [\frac{1}{2} ( Q_{\phi_a}\left(s_{t},a_t, z_t\right) - \bar{Q}_a )^2 ]$ \\ \COMMENT{update LL critic weights}
\STATE $\alpha_a \leftarrow \lambda_{\alpha_a}\big[\alpha_a( D_{KL}(\pi_{\theta_a}(a_t|s_t,z_t)\| p_{\bar{\psi}_a}(a_t|s_t,z_t))  - \delta_a)\big]$ \\ \COMMENT{update LL alpha} 
\STATE $\bar{\phi}_a \leftarrow \tau \phi_a + (1-\tau)\bar{\phi}_a$  \COMMENT{update LL target network weights}
\ENDFOR
\STATE \textbf{Return} trained low-level policy $\pi_{\theta_a}$
\end{algorithmic}
\end{algorithm}

 
% Equation~\eqref{Eqn: Qat} is inspired by the relationship between Q-functions between Q-functions on the semi-MDP \eqref{Eqn: Qa_noreg_b0} and \eqref{Eqn: Qa_noreg_b1}.  


% \subsubsection{Skill-Critic} %\label{subsec:skillcriticalgo}
% The complete algorithm is summarized in Algorithm~\ref{Alg:skill-critic-summary}.
% After a skill embedding and prior are learned from demonstrations (Section~\ref{Sec:skillprior}), Skill-Critic uses the incomplete skill set to train the HL and LL policies. 
% Rollouts are collected from the environment by sampling the HL policy every $H$ steps, and executing the selected skill for $H$ steps by sampling the LL policy.
% The action is executed in the environment, and $\{s,z,a,r,s'\}$ is stored. 
% Policy improvement occurs in two stages. 
% The HL policy, $\pi_z$ is optimized on $M^\mathcal{H}$ using critics $Q_{\phi_z}$ and $Q_{\bar{\phi}_z}$, and temperature parameter $\alpha_z$ (Line 9) via SPiRL~\cite{pertsch2021accelerating}. The LL policy, $\pi_a$, is optimized on $M^\mathcal{L}$ using critics $Q_{\phi_a}$ and $Q_{\bar{\phi}_a}$, and $\alpha_a$ (Line 11) via Algorithm~\ref{Alg:low-level}. 

% Unlike previous works that fixed the LL policy during training (i.e. $\pi^\mathcal{L}\doteq p_{\bar{\psi}_a}$) \cite{pertsch2021accelerating}, the RL fine-tuning of $\pi^\mathcal{L}=\pi_{\theta_a}$ with initial policy $\pi_{\theta_a}^0=p_{\bar{\psi}_a}$ allows us to \textit{improve} skills to maximize rewards. 

% \subsection{Skill Discovery} \label{Subsec: SkillDisc}
% \commentc{I think this can be moved to the appendix. it is an implementation detail. Also I would not say you "add"  a variance head, because really you are just initializing a stochastic policy's weights with the  weights of the decoder, right?}
% The Skill-Critic agent discovers new skills by exploring and updating low-level action policies. However, the low-level policy has the same structure as the decoder and only outputs deterministic actions, limiting exploration efficiency. To this end, we adopt a common strategy for continuous action exploration \textemdash probabilistic policy with variance. We add another variance head to the policy network to simultaneously generate the mean and standard deviation $\{\mu, \sigma \} \sim \pi^a_{\phi}$ and formulate them to a Gaussian distribution $\mathcal{N}(\mu, \sigma)$. We manually initialize the value of the variance head $\sigma_0$ to keep a moderate speed of skill exploration and update.

% \begin{equation} \label{Eqn: DKL_LL}
%     D_{K L}  \left(\pi^a_{\phi}\left(a_{t} \mid s_{t}, z_i, \bar{k}_{t}\right) \|  p_\phi\left(\hat{a}_{t} \mid s_{t}, z_i, \bar{k}_{t}\right)\right)  = D_{K L}\left( \mathcal{N}( \mu_{t}, \sigma_t ) \| \mathcal{N}(\hat{\mu}_{t} ,\sigma_0) \right)
% \end{equation}

% In Eqn.~\eqref{Eqn:LL obj}, the KL divergence of low-level policy constraints the distribution difference with the decoder. In practice, we also consider the variance head and derive the calculation in Eqn.~\eqref{Eqn: DKL_LL}, where $\{\mu_{t}, \sigma_t\}$ are output from the mean and variance heads of the policy network, while only the mean $\hat{\mu}_{t}$ is output by the decoder network and the variance $\sigma_0$ is still the initial value. So we constrain the low-level policy with the decoder output and the expected variance. We control the magnitude of KL divergence by setting a target value $\delta$ and use an auto-tuning strategy in (ref SPiRL) to regularize $\alpha$ and guide the policy convergence.





==> submit2/sections/conclusion.tex <==
% ============== conclusion =============
\section{Conclusion} \label{Sec:Conclusion}
We proposed Skill-Critic, a hierarchical skill-transfer RL algorithm, to perform two parallel policy optimization updates for skill selection and skill fine-tuning. We show that Skill-Critic can effectively leverage low-coverage and low-quality demonstrations to accelerate RL training, which is difficult with existing skill-transfer RL methods with stationary LL policies. In our experiments, our method solves maze navigation tasks that require exploring new skills online. Also, Skill-Critic outperforms existing methods on a challenging sparse-reward autonomous racing task and robotic manipulation task with the help of low-quality, non-expert demonstrations. 


\textit{Limitations and Future Work:} Skill-Critic reformulates hierarchical RL as two parallel MDPs. Alternating between HL and LL optimization does not guarantee an optimal joint policy for the original semi-MDP. In future work, we are interested in alternative theoretical frameworks to jointly optimize HL and LL policies for a single KL-regularized semi-MDP.  Further, we plan to alleviate the restriction of fixed skill horizons with adaptive horizons and explore frameworks that differentiate between skill improvement and skill discovery.


==> submit2/sections/experiments.tex <==

% =============== experiments ===========
\section{Experiments} \label{Sec:Exp}
% Our experiments aim to answer: (1) Can Skill-Critic effectively leverage low-coverage, low-quality demonstrations to accelerate downstream RL? (2) Is the proposed LL policy update step necessary in improving the skill set and optimizing the agent performance in the downstream task?  

 We assess Skill-Critic in three tasks: maze navigation, racing, and robotic manipulation (Fig. \ref{fig:all_tasks}). Please refer to our websites for demo videos. In each task, Stage 1 consists of collecting an offline dataset to create an informative skill set; however, it may not encompass \textit{all} of the skills necessary for downstream tasks. Stage 2 consists of a sparse-reward episodic RL task. A binary reward (+1) is received at each time step after the goal is reached. The objective is to maximize the sum of rewards, i.e. complete the task \textit{as fast as possible}.

We compare Skill-Critic to several baselines. \textbf{SPiRL}~\cite{pertsch2021accelerating} extracts temporally extended skills with a skill prior from offline data, but downstream RL training occurs only on the HL skill selection policy. Our version of SPiRL uses a state-dependent policy to improve performance~\cite{pertsch2021guided}. Our \textbf{Skill-Critic} is warm-started with SPiRL at $N_{\textrm{HL-warm-up}}$ steps to stabilize the HL policy prior to LL policy improvement. 
\textbf{ReSkill}~\cite{rana2023residual} is a HRL method that uses residual skill policies to augment the stationary LL policy. This contrasts Skill-Critic, which directly fine-tunes the nonstationary LL policy with regularization to the stationary action prior.
  ReSkill\footnote{As this work focuses on the parallel policy update, for Maze and Racing tasks, our ReSkill implementation employs an identical Stage 1 skill embedding to SPiRL \cite{pertsch2021accelerating}, but the HL and LL policy updates are the same as ReSkill \cite{rana2023residual}. We provide the best hyperparameters for the weight of the residual policy in the supplemental code. The robotic task employs the identical implementation as \cite{rana2023residual}.} uses independent HL and LL policy updates, but Skill-Critic relates the LL Q-function to the HL Q-function upon arrival at the next skill~\eqref{Eqn: Qatau}. 
Baselines also include soft actor-critic (\textbf{SAC})\cite{haarnoja2018soft} and SAC initialized with behavioral cloning~(\textbf{BC+SAC}).

 % We evaluate the environment reward, to test not only whether the task is completed, but also how well the task is completed. 


\subsection{Maze Navigation and Trajectory Planning}
The maze task tests if Skill-Critic can improve its LL policy and leverage the action prior to learn challenging, long-horizon tasks.
The task uses the D4RL point maze~\cite{fu2020d4rl} with a top-down agent-centric state and continuous 2D velocity as the action. Demonstrations consist of 85000 goal-reaching trajectories in randomly generated, small maze layouts (Fig.~\ref{fig:all_tasks}a). The demonstration planner~\cite{pertsch2021accelerating} acts in right angles (i.e. the demonstrator goes up, down, left or right). 
% In Stage 1, the agent can learn skills such as traversing hallways or passing through doors.
% that it can transfer to Stage 2. 
For Stage 2 downstream learning, we introduce two new maze layouts: 1.) a \textit{Diagonal Maze} to test how well the agent can navigate a maze with unseen passageways, and 2.) a \textit{Curvy Tunnel} with multiple options for position, heading, and velocity to test how well the agent can plan an optimal trajectory. In both layouts, the agent has 2000 step episodes and receives a $+1$ reward for each time step that the distance to the goal is below a threshold. Unlike SPiRL \cite{pertsch2021accelerating}, in our maze layouts, the agent can significantly improve its performance by moving diagonally and following a smooth path.


% We aim to test whether Skill-Critic can accelerate downstream RL using offline demonstrations and improve task performance with the LL policy update. 


In both maze tasks in Fig. \ref{fig:MazeResults}, SAC and BC+SAC fail to reach the goal, likely because the single-step policy cannot discover the sparse reward. Although ReSkill leverages the skill embedding to guide exploration, the LL residual policy update is independent of the HL update, and ReSkill eventually fails to reach the goal. Noting the maze tasks have a longer horizon than the robotic tasks \cite{rana2023residual}, we hypothesize the distant goal's reward signal is too weak to guide the LL residual policy (see ablation in Section \ref{sec:LLQablation}).  In contrast, SPiRL and Skill-Critic use the offline demonstrations and $H$-step reward to reach the goal. Fig. \ref{fig:MazeResults} compares the trajectories of Skill-Critic and SPiRL. SPiRL plans slow, jagged trajectories because it cannot improve the offline-learned LL policy.   Skill-Critic updates the LL policy to further optimize its path, resulting in planning a significantly faster trajectory.  Interestingly, Skill-Critic \textit{discovers} diagonal motion, but it still does not forget to solve the maze because LL policy exploration is guided by the action prior.

% (see ablations in Section \ref{subsec: ablation}).
% (ablations in Appendix~\ref{Appendix: Ablation}).

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.27\textwidth,trim={0 0pt 0 0pt},clip]{figures/env1_cropped.pdf}
%     \caption{Maze Tasks. Stage 1 demonstration uses the planner in SPiRL \cite{pertsch2021accelerating}. We create two complicated stage 2 RL tasks to test the agent's navigation in a \textit{Diagonal Maze} (left) and path planning in a \textit{Curvy Tunnel} (right).}
%     \label{fig:env_maze}
% \end{figure}
% \begin{figure*}[t]
%     \centering
%         \includegraphics[width=0.32\textwidth]{figures/maze.pdf}
%     \includegraphics[width=0.30\textwidth,trim={25cm 0 0 0},clip]{figures/MazeExp.pdf}
%     \caption{Maze task results. \textbf{Left:} mean (std) episode rewards with 3 random seeds. Skill-Critic begins training at 1 million steps and is warm-started by SPiRL.\textbf{Right:} Trajectories after policies converge. SPiRL reuses right-angle skills, but Skill-Critic discovers new skills to plan  diagonal and curved paths.}
%     \label{fig:MazeResults}
% \end{figure*}
\begin{figure*}[t]
    \centering
    \subfigure[\textit{Diagonal Maze} \& \textit{Curvy Tunnel} Maze Tasks]{\makebox[.33\textwidth]{\includegraphics[width=.27\textwidth,trim={0 0pt 0 0pt},clip]{figures/env1_cropped.pdf}}}\hfill
        \subfigure[Gran Turismo Sport (GTS) Racing Task]{\makebox[.3\textwidth]{
    \includegraphics[width=0.27\textwidth]{figures/env2_cropped.pdf}}}\hfill
        \subfigure[7DoF Robotic Manipulation Tasks ]{\makebox[.27\textwidth]{
    \includegraphics[width=.27\textwidth]{figures/env3_cropped.pdf}}}
        \caption{Demonstrations and experiments. (a) Maze Tasks: Stage 1 demonstration uses the planner in SPiRL \cite{pertsch2021accelerating}. Stage 2 tasks test the agent's navigation in a \textit{Diagonal Maze} and path planning in a \textit{Curvy Tunnel}. (b)  GTS Racing on a single corner. The agent achieves +1 after the goal state is passed. Demonstrations start at random low-speed starting points on the course. (c) Robotic Manipulation: Stage 1 demonstrations use a hand-crafted controller \cite{rana2023residual} to push a block across a table. Stage 2 RL tasks are \textit{Slippery Push}, which uses a more slippery surface, and \textit{Cleanup Table}, which includes a tray as an obstacle.}
    \label{fig:all_tasks}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth, trim={0.25cm 9pt 0 3pt},clip]{figures/maze2.pdf}
    \hspace{-1cm}
    \includegraphics[width=0.195\textwidth,trim={0 0 0 0},clip]{figures/MazeExp2_1.pdf}
    % \subfigure[Mean (std) episode rewards (5 seeds)]{
    %     \includegraphics[width=0.25\textwidth, trim={0.25cm 0 0 0},clip]{figures/maze2.pdf}}
    %         % \subfigure[Policy Trajectories]{\raisebox{0.35em}{
    % % \includegraphics[width=0.2\textwidth,trim={25cm 0 0 0},clip]{figures/MazeExp.pdf}}}
    %             \subfigure[Policy Trajectories]{\raisebox{0.65em}{
    % \includegraphics[width=0.2\textwidth,trim={0 0 0 0},clip]{figures/MazeExp2_1.pdf}}}
    \caption{Maze results. \textbf{Left:} Rewards. Skill-Critic starts training at $N_{\textrm{HL-warm-up}}$=1M steps. \textbf{Right:} Trajectories after policies converge. SPiRL reuses right-angle skills, but Skill-Critic plans diagonal and curved paths. }
    \label{fig:MazeResults}
\end{figure}

% \chen{It looks quite messy. If you want to save space, consider putting the three task figures (maze, GTS, robotics) side-by-side as three subplots.}






\subsection{Autonomous Racing}
The vehicle racing task tests if Skill-Critic can 1.) improve the LL policy when there is only access to low-coverage, low-quality demonstrations, and 2.) leverage the skill and action prior to accelerate learning a sparse reward.
We employ the Gran Turismo Sport (GTS) high-fidelity racing simulator to solve a new, sparse-reward racing task. The low-dimensional state \cite{fuchs2021super} includes pose, velocity, and track information. There are two continuous actions: steering angle and a combined throttle/brake command between $[-1,1]$. The agent starts at a low speed in the center of the track and has 600-step (60-sec) episodes; the agent receives a binary +1 reward at each time step after it passes the goal.  
We use GTS's Built-in AI controller to collect 40000 \textit{low-speed} demonstrations from random starting points on the course, each 200 steps in length. The agent can transfer skills such as speeding up and turning but must drive at higher speeds to rapidly navigate the course.

\begin{figure}[t]
    \centering
\subfigure[Episode rewards and hit wall time during training]{
    \makebox[\columnwidth]{\includegraphics[width=.97\columnwidth, trim={0pt, 9pt, 0, 3pt}, clip]{figures/gts_no_traj.pdf}}  }
    \subfigure[Time to finish course at convergence]{ \begin{minipage}{\columnwidth}
    \centering
            \scriptsize
            \begin{tabular}{|c|c|}
                \hline
                \textbf{Algorithm} & \textbf{Finish Time (s)} \\
                \hline  
                Skill-Critic & 27.2$\pm$0.6 \\
                ReSkill & 29.9$\pm$0.2\\
                SPiRL & 36.4$\pm$0.9\\
                \hline
            \end{tabular}
                        \begin{tabular}{|c|c|}
                \hline
                \textbf{Algorithm} & \textbf{Finish Time (s)} \\
                \hline  
                BC+SAC & 59.6$\pm$0.7\\
                SAC & 56.8$\pm$2.9 \\
                \hline
                \textit{Built-In AI} & 26.1\\
                \hline
            \end{tabular}
            \vspace{3pt}
        \end{minipage}}
    \caption{GTS Racing Results. \textbf{Left:} mean (std) episode reward. \textbf{Right:} mean (std) of cumulative time in contact with track boundary per episode. SPiRL does not improve, so Skill-Critic does not use warm-up: $N_{\textrm{HL-warm-up}}=0$.}
    \label{fig:RaceResults}
\end{figure}


 We compare performance to GTS's Built-in AI, which is a high-quality, rule-based controller deployed with the game as a competitor for players.
 Note that we deliberately give Skill-Critic access to low-speed demonstrations from Built-in AI to test Skill-Critic's ability to improve skills. Unlike previous works in GTS with dense rewards that must be uniquely designed for each car and track~\cite{fuchs2021super, wurman2022outracing}, we use a generalizable sparse reward in a single corner (Fig.~\ref{fig:all_tasks}b). Given these factors, we consider Built-in AI a strong baseline. 


% and also consider GTS's Built-in AI as a strong baseline. 
% The Built-in AI is a high-quality, rule-based controller deployed with the game as a competitor for players. 
% We compare  trajectories from each method's highest reward policy. 

% The baselines fail to efficiently solve sparse-reward racing.
In Fig.~\ref{fig:RaceResults}, we compare (a) rewards, which indicates how fast the car completes the course, and time in contact with the wall at the edge of the track, which indicates the car's dynamic stability, and (b) the converged policy's time to finish the corner.
 SAC reaches the goal in spite of its single-step policy, but it is slow to improve with the sparse reward. BC+SAC appears to hinder exploration, consistently crashing in the first straight-away.
In contrast, SPiRL exploits the pre-trained skills to reach the goal. However, skills are learned from low-speed demonstrations, so the stationary LL policy may only be capable of low-speed maneuvers. 
% SPiRL's stationary LL policy may suffer from distributional shifts if the demonstrations are not sufficient to cover the vehicle dynamics at unseen states. 
Thus, SPiRL cannot plan high-speed trajectories and collides with the wall. 



Both Skill-Critic and ReSkill address these issues to achieve high rewards and reduce contact time with course walls. Both methods exploit offline pre-training and temporally extended actions to guide exploration and maintain knowledge of the sparse reward. Also, online LL fine-tuning is critical to learn high-velocity maneuvers, such as collision avoidance and sharp cornering. However, ReSkill's LL residual policy update, which is independent of the value assigned by the HL update, does not improve the LL policy at states early in the rollout, resulting in a lower finish time. Conversely, Skill-Critic races close to the speed of the Built-in AI. We attribute this to the interrelated Q-function update that estimates the LL Q function using the $H$-step reward  \textit{upon arrival} to a skill. As shown in~\ref{sec:LLQablation}, sparse rewards propagate further into the LL policy update, yielding higher state values. As shown in the demo videos, SPiRL is slow and collision-prone, and ReSkill yields frequent oscillation. In contrast, Skill-Critic is able to drive the race car in a faster and more stable manner. 

%Despite the sparse reward and low-speed demonstrations, Skill-Critic is the only learned policy that can consistently perform as well as the Built-in AI.

\subsection{Robot Manipulation} Finally, we test a sparse-reward robot manipulation task with a 7-DoF Fetch robotic arm simulated in MuJoCO \cite{todorov2012mujoco}. Handcrafted controllers \cite{rana2023residual} collect 40k demonstration trajectories, where the robot must \textit{Push} a block along a table (Fig.~\ref{fig:all_tasks}c).
For the Stage 2 RL tasks, we test \textit{Slippery Push} and \textit{Cleanup Table} tasks \cite{rana2023residual}.
In \emph{Slippery Push} the agent must push a block to a goal 100 step episodes, but the friction of the table surface is reduced from that seen in the demonstrations. The agent receives a reward of 1 once the block is at the goal location, otherwise the reward is 0; episodes are 100 steps. 
For \emph{Cleanup Table} task, the agent must place a block on a rigid tray object, which was not present in the demonstrations. The agent receives a reward of 1 only when the block is placed on the tray, otherwise the reward is 0; episodes are 50 steps. 

\begin{figure}[t]
    \centering
    % \caption{Robotic task.  }
%     \label{fig:env_robot}
% \end{figure}
% \begin{figure}[t]
%     \centering
        \makebox[\columnwidth]{
    \includegraphics[width=.97\columnwidth, trim={0pt, 9pt, 0, 3pt}, clip]{figures/robot.pdf}}
    % \includegraphics[width=.47\columnwidth]{figures/cleantable.pdf}}}
    \caption{Robotic Manipulation results.  Mean episode reward (std). Skill-Critic employs $ N_{\textrm{HL-warm-up}}$=500k steps. Left: Slippery Push, Right: Cleanup Table }
    \label{fig:fetchresults}
\end{figure}



ReSkill outperforms other hierarchical methods like Hierarchical Actor Critic (HAC) \cite{levy2018learning} and PARROT \cite{singh2020parrot}, which do not learn anything meaningful (see results in \cite{rana2023residual}). In comparison to SPiRL and Skill-Critic (Fig. \ref{fig:fetchresults}), ReSkill speeds up exploration with its alternative skill embedding that biases the HL policy towards relevant skills. However, Skill-Critic achieves a higher reward by completing the task even \textit{faster}. As shown in the demo videos, ReSkill corrects SPiRL's pre-trained policy that aggressively pushes the block, but Skill-Critic is the fastest to push the block to the goal.   Interesting future research could apply ReSkill's alternative skill embedding to Skill-Critic, but we believe Skill-Critic's LL policy update is crucial to converge to the highest reward.
 % ReSkill's LL residual policy updates with the single-step reward $r(s,a)$. 

 % We attribute this to the interrelated Q-function update that estimates the LL Q function using the $H$ step reward estimate \textit{upon arrival} to a skill. As shown in~\ref{sec:LLQablation}, this allows sparse rewards to propagate further into the LL policy update, resulting in higher state values.

\subsection{Ablation Studies}

\begin{figure}[t]
\centering
        \raisebox{0.95em}{\includegraphics[width=.25\textwidth]{figures/m2_independent.pdf}}
        \includegraphics[width=.135\textwidth]{figures/Qa2.pdf}
    \caption{Ablation of $Q^a$ update in \textit{Curvy Tunnel} ($N_{\textrm{HL-warm-up}}$=1M, 3 seeds). \textbf{Independent} update of $Q^a_{\beta(s_{t+1})=1}$ from current $Q^a$ estimate versus \textbf{Skill-Critic} update of $Q^a_{\beta(s_{t+1})=1}$ from current $Q^z$ estimate. \textbf{Left}: training episode rewards.
    \textbf{Right:} value distribution of trajectories at convergence.}
    \label{Fig: Qa_ablation}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[Ablation: Prior Distribution]{\includegraphics[width=0.235\textwidth]{figures/m2_flatprior_rew.pdf}}
        \subfigure[Ablation: Action Prior Variance]{\includegraphics[width=0.235\textwidth]{figures/m2_var_rew.pdf}}
            % \includegraphics[width=0.5\textwidth,trim={12.5cm 0 0 0},clip]{figures/Ablation.pdf}
            \subfigure[Ablation Study of KL Divergence]{\includegraphics[width=.485\textwidth]{figures/m2_td.pdf}}
    \caption{Ablation studies of LL policy regularization in \textit{Diagonal Maze} ($N_{\textrm{HL-warm-up}}=1$M, 3 seeds). \textbf{(a):} LL policy prior distribution: uniform prior (entropy) or proposed nonuniform prior (KL divergence).  \textbf{(b):} Variance of the action prior, $\sigma_{\hat{a}}$. \textbf{(c)}: LL policy target KL divergence, $\delta_a$, training rewards (left) and actual KL divergence during training (right).}
    \label{fig:LLablation}
\end{figure}

\subsubsection{LL Q Function Estimate}\label{sec:LLQablation}
\textbf{Skill-Critic} uses the value \textit{upon arrival} to a new skill to estimate $Q_a$ by using $Q_{\bar{\phi}_z}$(Line 4 of Algorithm \ref{Alg:low-level}). 
Namely, when $\beta(s_{t+1})=0$, $Q^a$ is estimated with single-step discounting \eqref{Eqn: Qatau}, but when $\beta(s_{t+1})=1$, $Q^a$  is estimated with $H$-step discounting \eqref{Eqn: Qat}.
In Fig. \ref{Fig: Qa_ablation}, we compare this to ``independent'' estimation of $Q^a$ and $Q^z$ in \textit{Curvy Tunnel}. \textbf{Independent} refers to estimating $Q^a$ with~\eqref{Eqn: Qatau} regardless of the value of $\beta(s_{t+1})$. 
% \textbf{Skill-Critic} refers to the $Q^a$ estimate described in Algorithm \ref{Alg:low-level}. 
The high-MDP policy, $\pi_z$, and critic, $Q^z$, are warm-started for 1M steps of SPiRL, then $\pi_a$ and $\pi_z$ are trained (Algorithm \ref{Alg:skill-critic-summary}) for an additional 1M steps. In Fig. \ref{Fig: Qa_ablation}, the \textbf{independent} LL Q-value hinders exploration, and eventually, the policy can no longer find the goal. We hypothesize the distant goal's reward signal is too weak to guide the policy at states early in the roll-out due to single-step exponential discounting~\eqref{Eqn: Qatau} even for larger values of $\gamma$.
\textbf{Skill-Critic} includes $Q^z$ in the estimate of $Q^a$, with two benefits: 1) the $H$ step discounting of $Q^z$ is less prone to losing the sparse reward signal at early states, and 2) the LL policy update uses state-skill values assigned by the HL policy. The ablation also informs why $N_{\textrm{HL-warm-up}}>0$ is necessary for success in the maze and robot tasks, as HL warm-up allows accurate $Q^z$ estimates.
% Thus, Skill-Critic outperforms independent Q-function estimation to consistently reach the goals.






% $^1$\footnote{$^1$To further comment on point 2: we have formulated $M^\mathcal{H}$ and $M^\mathcal{L}$ as two separate, parallel optimization problems. In theory, separate samples and convergence should be acquired before changing between the HL and LL problems, but Skill-Critic uses the same samples and single steps on each optimization problem, following the precedent in options frameworks \cite{zhang2019dac}. Intuitively, including $Q^z$ in the update of $Q^a$ may better link the parallel optimization problems, although future work is needed to show the exact mechanism and effect of this link.}
% Due to this desirable performance, we employ the \textbf{Skill-Critic} update for the rest of the experiments in this paper.

% In contrast, the 
% \textbf{Skill-Critic} LL Q-function update uses When $\beta(s_{t+1})=0$, estimation of $Q^a$ still relies on single-step discounting for LL policy refinement. However, when $\beta(s_{t+1})=1$, the current skill, $z_t$, is finished and a new one will be selected in the next time step. Here, when $\beta(s_{t+1})=1$, Skill-Critic employs Eqn. \eqref{Eqn: Qat} to estimate the current value of the skill. 

% The results suggest that the independent LL Q-value hampers exploration, leading to a rapid decline in episode returns, possibly because the distant goal's reward signal is too weak for earlier state guidance due to exponential discounting. In contrast, the Skill-Critic LL Q-value, incorporating $Q^z$ value, maintains exploration and rewards improvement without losing goal-finding ability. When $\beta(s_{t+1})=0$, $Q^a$ relies on single-step discounting, but with $\beta(s_{t+1})=1$, Skill-Critic employs Eqn. \eqref{Eqn: Qat} to estimate skill value. This benefits by 1) applying $H$-step discounting for HL Q-value ($Q^z$), capturing longer-horizon rewards better, and 2) informing the LL policy update with state-skill values from the HL policy. Due to these advantages, we exclusively use the Skill-Critic update for the remaining experiments in this paper.

\subsubsection{LL Policy Regularization}
Fig. \ref{fig:LLablation}, provides an ablation on LL policy regularization in \textit{Diagonal Maze}. All methods use $N_{\textrm{HL-warm-up}}=1$M, then are trained via Skill-Critic with the specified hyperparameter. 
In Fig. \ref{fig:LLablation}(a), we replace Skill-Critic's non-uniform action prior divergence term with a LL policy update with a uniform prior \cite{haarnoja2018soft}, which is identical to entropy regularization~\cite{pertsch2021accelerating}.  A uniform prior leads to poor exploration, as entropy encourages random actions that are not guided to the sparse reward. Fig. \ref{fig:LLablation}(b) changes variance of the action prior, $\sigma_{\hat{a}}$, which determines policy variation from the pre-trained decoder (\ref{Sec:skillprior}). Small values (e.g. $\log \sigma_{\hat{a}}=-5$), over-constrain the LL policy. However, with large variance, e.g. $\log \sigma_{\hat{a}}=-1$, the agent forgets the pre-trained skills. A suitable value is $\log \sigma_{\hat{a}}=-3$, which promotes exploitation of the decoder and exploration to improve skills.
 In Fig. \ref{fig:LLablation}(c) we compare rewards for varying values of $\delta_a$ and the actual KL divergence of the LL policy from the action prior during training. As explained in Algorithm \ref{Alg:low-level} [Line 9], $\alpha_a$ is a dual descent parameter to constrain the LL policy's divergence to the target divergence $\delta_a$ \cite{haarnoja2018soft, pertsch2021accelerating}. As  $\delta_a$ increases, rewards likewise increase as the LL policy has freedom to deviate from the action prior. The LL policy divergence does converge to $\delta_a$, but in early training (<.2M steps), KL divergence is relatively low for the initial $\alpha_a$ in \cite{pertsch2021accelerating, haarnoja2018soft}. Thus, the initial $\alpha_a$ may also be an important hyperparameter for stable training.
 % Conversely, a smaller target divergence constrains the policy closer to the action prior, and Skill-Critic receives less reward. 




==> submit2/sections/experiments_archive.tex <==

% =============== experiments ===========
\section{Experiments} \label{Sec:Exp}
Our experiments aim to answer: (1) Can Skill-Critic effectively leverage low-coverage, low-quality demonstrations to accelerate downstream RL? (2) Is the proposed LL policy update step necessary in improving the skill set and optimizing the agent performance in the downstream task?  

% ===================== env intro ================
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.76942\textwidth]{figures/EnvFigs2.pdf}
    \caption{For each environment, we collect an offline dataset for skill training (\textbf{left}), and test skill improvement on more complex target tasks (\textbf{right}). The agent must use short navigation skills to guide it through a diagonal maze or complicated trajectory planning (\textbf{top}), and use low-velocity trajectories to navigate a corner of the racetrack as quickly as possible (\textbf{bottom}).}
    \label{fig:EnvFigs}
\end{figure*}

\begin{figure}[t]
    \centering
    \subfigure[Table Cleanup]{
    \includegraphics[width=.45\columnwidth]{figures/slipperpush.png}}
        \subfigure[Slippery Push]{
    \includegraphics[width=.45\columnwidth]{figures/slipperpush.png}}
    \caption{\textbf{\color{black}{Robotic Arm Evaluation Environment}}\color{black}{ proposed by Rana et al \cite{rana2023residual}. A MuJoCO-based \cite{todorov2012mujoco} 7-DoF Fetch robotic arm interacts with objects placed in front of it to place a block on a tray in the scene (Table Cleanup) or push a block along a slippery table to a goal (Slippery Push).}}
    \label{fig:fetcharm}
\end{figure}

\subsection{Environments, Tasks, and Demonstrations} \label{Subsec: Exp env} We evaluate Skill-Critic in three tasks: maze navigation, maze trajectory planning, and autonomous racing (Fig.~\ref{fig:EnvFigs}). We collect a large dataset of demonstrations that can create an informative skill set; however, the skill set does not contain \textit{all} of the potential skills that may aid downstream tasks. We evaluate the environment reward, to test not only whether the task is completed, but also how well the task is completed.
% instead of a simple task success rate. 

% Appendix~\ref{Appendix: env} contains a full description of environments and data collection.

{\bf Maze Navigation.}
The maze navigation task is based on the D4RL point maze environment~\cite{fu2020d4rl} that uses a top-down agent-centric state and 2D velocity as the action. We use the same planner-based demonstrations as~\cite{pertsch2021accelerating}, consisting of 85000 goal-reaching trajectories in randomly generated, small maze layouts. We create a new maze navigation task with multiple diagonal tunnels (see Fig.~\ref{fig:EnvFigs}) for downstream learning. The agent has 2000 steps in each episode and receives a binary reward for each time-step that the distance to the goal is below a threshold, encouraging the agent to reach the goal in fewer steps. The agent can transfer skills such as traversing hallways or passing through doors.
% , but must learn to rapidly navigate the diagonal maze. 
% The state consists of an RGB top-down view centered around the agent augmented with the time since the last skill was completed, $k$.


{\bf Maze Trajectory Planning.}
The maze trajectory planning task uses the same skills, simulation engine, episode length, and reward as the maze navigation task. The difference is that the downstream environment has a curvy tunnel with corners of varying shapes, offering the agent multiple options for position, heading, and velocity.  To minimize time to reach the goal, the agent must learn to create 
a smooth trajectory specialized to the full course.

\begin{newtext}
\textbf{Robot Manipulation: } We implement robot manipulation experiments on a 7-DoF Fetch robotic arm simulated in MuJoCO \cite{todorov2012mujoco}. We directly use two tasks proposed in Rana et al. \cite{rana2023residual} as shown in Fig. \ref{fig:fetcharm}. We use the demonstration data consisting of 40k trajectories provided by Rana et al. \cite{rana2023residual}, which was collected with handcrafted controllers. 
For \emph{Slippery Push} task, the agent is required to push a block to a given goal, but the friction of the table surface is lowered from that seen in the demonstrations. The agent receives a reward of 1 once the block is at the goal location, otherwise the reward is 0. The task is episodic and terminates after 100 steps. 
For \emph{Table Cleanup} task, the agent must place a block on a rigid tray object, which was not present in the demonstrations. The agent receives a reward of 1 only when the block is placed on the tray, otherwise the reward is 0. The task is episodic and terminates after 50 steps.
\end{newtext}

{\bf Autonomous Racing.}
We employ the Gran Turismo Sport (GTS) high-fidelity racing simulator~\cite{fuchs2021super} to test a new, sparse reward autonomous racing task. The low-dimensional state representation includes pose, velocity, and track information. There are two continuous actions: steering angle and a combined throttle/brake command between $[-1,1]$. Unlike previous works in GTS~\cite{fuchs2021super, wurman2022outracing}, we create a sparse reward to navigate a single corner. The agent starts at a low speed in the center of the track and has 600-step (60-sec) episodes; the agent receives a binary +1 reward for every time step when it passes the finish line.  For demonstrations, we use GTS's built-in AI controller to collect 40000 trajectories from random, low-speed starting points on the course, each 200 steps in length. While the built-in AI is capable of controlling the race car at high-speed, we deliberately bias the demonstration toward low-speed maneuvers to test Skill-Critic's ability to improve skills. The agent can transfer skills such as speeding up and turning from the low-speed demonstrations but must improve these skills to complete the corner as fast as possible.
% In the downstream RL task, suboptimal skills hinder fast and collision-free trajectory planning. These demonstrations navigate the corner, but are suboptimally slow.

{\bf Baselines.} We compare Skill-Critic with existing methods to show the necessity of fine-tuning a temporally abstracted LL policy. \textbf{SAC} performs model-free RL via SAC~\cite{haarnoja2018soft} without offline experience or temporal abstraction. \textbf{BC+SAC} uses offline experience to initialize a policy with behavioral cloning (BC), then fine-tune the policy via SAC. \textbf{SPiRL}~\cite{pertsch2021accelerating} extracts temporally extended skills with a skill prior from the offline data, but downstream RL training occurs only on the HL skill selection policy. Our version of SPiRL uses a state-dependent policy to improve performance~\cite{pertsch2021guided}. 
\begin{newtext}
\textbf{ReSkill}~\cite{rana2023residual} is a hierarchical RL method that uses residual skill policies to augment the stationary LL policy during training rather than directly fine-tuning the learned LL policy.
\end{newtext}

% =============== main results ==============




\subsection{Experimental Results} \label{Subsec: ExpMazeNav}

{\bf Maze Navigation and Trajectory Planning.} 
We analyze the maze tasks in Figure~\ref{fig:MazeResults}. In both tasks, SAC and BC+SAC fail to reach the goal, likely since the single-step policy is unable to discover the sparse reward. In comparison, the temporally abstracted methods (SPiRL and Skill-Critic) can effectively utilize offline demonstrations to successfully find and reach the goal. However, SPiRL plans slow, jagged trajectories because it cannot improve the offline-learned skills. We warm-start Skill-Critic with SPiRL after 1M steps to stabilize the HL policy, and Skill-Critic is then able to further optimize its path, resulting in planning an optimal trajectory. Skill-Critic \textit{discovers} diagonal motion, but it does not forget the skills to solve the maze due to the LL policy regularization. This regularization is crucial to  guide exploration.
% (ablations in Appendix~\ref{Appendix: Ablation}).

\begin{figure*}[t]
    \centering
        \includegraphics[width=0.4\textwidth]{figures/maze.pdf}
    \includegraphics[width=0.4\textwidth,trim={25cm 0 0 0},clip]{figures/MazeExp.pdf}
    \caption{Maze experiment results. \textbf{Left:} average episode rewards with 3 random seeds. Skill-Critic begins training at 1 million steps and is warm-started by SPiRL. \textbf{Right:} SPiRL and Skill-Critic trajectories at convergence. SPiRL reuses right-angle movements from the skills, resulting in slow, jagged paths. Skill critic discovers new skills to plan diagonal trajectories.}
    \label{fig:MazeResults}
\end{figure*}

\begin{newtext}
{\bf Robot Manipulation}. We provide the results for the 7-DoF Fetch arm tasks in Fig. \ref{fig:fetchresults}. As originally shown in the original paper \cite{rana2023residual}, ReSkill quickly learns a policy to clean the table, and outperforms other hierarchical methods like Hierarchical Actor Critic (HAC) \cite{levy2018learning} and PARROT \cite{singh2020parrot}, which are unable to learn anything meaningful on the task (see results in \cite{rana2023residual}). The alternative skill-embedding space in ReSkill speeds up exploration by biasing the HL policy towards skills relevant to the state. However, the LL residual policy in ReSkill only improves its value through the single-step reward $r(s,a)$. Skill-Critic can achieve an even higher reward by completing the task even \textit{faster}. We attribute this to the inter-related Q-function update that estimates the LL Q-function using the $H$-step reward estimate \textit{upon arrival} to a skill (refer to \ref{Eqn: Qatau} and \ref{Eqn: Qat} in the text). Thus, the sparse reward is able to propagate further into the LL policy update, resulting in higher rewards. An interesting area for future research would be to apply ReSkill's alternative skill embedding to Skill-Critic to accelerate training.  However, we believe Skill-Critic's LL policy update is crucial to converge to the highest reward.
\end{newtext}

\begin{figure}[t]
    \centering
        \subfigure[Table Cleanup]{
    \includegraphics[width=.46\columnwidth]{figures/cleantable.pdf}}
            \subfigure[Slippery Push]{
    \includegraphics[width=.46\columnwidth]{figures/slippery_rew.pdf}}
    \caption{\textbf{\color{black}{Evaluation on 7DoF Robotic Arm. }} \color{black}{Mean episode reward (std) for each environment. Skill-Critic is warm-started with SPiRL at 500k steps.  Note how Skill-Critic achieves a higher reward.}}
    \label{fig:fetchresults}
\end{figure}

{\bf Autonomous Racing}. \label{Subsec: ExpRacing}
In Fig.~\ref{fig:RaceResults}, we evaluate the performance of RL training in the autonomous racing task using the episode reward and time in contact with the wall on the edge of the track. Further, we analyze the trajectories from each method's highest reward policy. 
SAC sufficiently explores to eventually reach the goal, but is slow to improve its policy with the sparse reward, resulting in policies with relatively low velocity. Warm-starting the SAC policy appears to hinder exploration; in fact, BC+SAC is unable to find the goal, and its trajectories consistently crash within the first straight-away.
In contrast, SPiRL makes use of the pre-trained skills, allowing it to exploit skills that can consistently reach the goal. However, these skills are learned from low-speed demonstrations. Thus, SPiRL's HL policy cannot generate high-speed trajectories given the stationary LL policy that is only capable of low-speed maneuvers. Plus, since the demonstration is limited in diversity, the offline learned skills suffer from distributional shifts. As a result, SPiRL frequently collides with the wall throughout the corner. All these factors prevent SPiRL from further improving its performance.

\begin{figure*}[t]
    \centering
    \includegraphics[width=.85\textwidth]{figures/gts_without_hitting_velocity.pdf}
    \caption{Autonomous racing results in Gran Turismo Sport. \textbf{Top left:} mean (std) episode reward. \textbf{Bottom left:} mean (std) of cumulative time in contact with wall at track boundary per episode (bottom). \textbf{Right:} Visualization of the trajectories from each method's highest scoring policy. Car markers indicate location at various times. Inset plot shows velocity vs. position along the track.}
    \label{fig:RaceResults}
\end{figure*}

Skill-Critic addresses these issues with online LL policy training, achieving higher episode rewards, reducing contact time with course walls, and quickly navigating the corner. Skill-Critic exploits the offline pre-training and temporally extended actions to guide exploration. Furthermore, the LL fine-tuning allows the Skill-Critic agent to navigate at a high velocity, which requires complex maneuvers like avoiding collision and slowing and turning hard in the corner. For reference, we compare the performance to GTS's Built-in AI, which is a high-quality, rule-based controller deployed with the game as a competitor for players. Note that Skill-Critic only has access to low-speed demonstrations from Built-in AI, and we use a \emph{sparse} reward, unlike previous methods with hand-engineered dense rewards~\cite{wurman2022outracing}. Given these factors, we consider Built-in AI a strong baseline for this single-corner racing task. Despite this, the Skill-Critic policy can consistently perform as well as the Built-in AI.

\begin{newtext}
    
\subsection{Ablation Study} \label{subsec: ablation}

\begin{figure}[t]
    \centering
   {\sffamily Target Divergence (td)}\\
    \includegraphics[width=.46\columnwidth,trim={0 0 24.5cm 1cm},clip]{figures/Ablation.pdf} \includegraphics[width=.46\columnwidth]{figures/maze2_KD.pdf}
    \caption{Ablation study of LL policy regularization in the Maze Navigation task. All agents are warm-started by SPiRL for 1 million steps. \textbf{Left:} LL policy target KL divergence, $\delta_a$. \textbf{\color{black}{Right:}} \color{black}{LL policy's actual KL divergence from the action prior during training.}}
    \label{fig:Ablation_kl}
\end{figure}

\begin{figure}[t]
    \centering
        \includegraphics[width=0.92\columnwidth,trim={12.5cm 0 0 0},clip]{figures/Ablation.pdf}
    \caption{Ablation study of LL action prior variance in the Maze Navigation task. All agents are warm-started by SPiRL for 1 million steps. \textbf{Left:} Prior distribution for LL policy regularization: uniform prior (entropy) or proposed non-uniform prior (KL divergence).  \textbf{Right:} LL policy initial variance, $\sigma_{\hat{a}}$. }
    \label{fig:Ablation}
\end{figure}

In this section, we examine the effect of the regularization for the LL policy and its effect on the overall performance of the skill critic algorithm. As we have described in Section \ref{Sec:HRLregularize}, the LL policy is regularized by the action prior, which is informed by the pre-trained decoder. 
In the experiments in Fig. \ref{fig:Ablation_kl} and Fig. \ref{fig:Ablation}, we demonstrate that it is necessary to regularize the LL policy with the action prior using KL divergence, and analyze the effect of related hyperparameters. 

\textbf{LL Target KL Divergence.} In Fig. \ref{fig:Ablation_kl}, we compare varying values for the low-level policy target KL divergence, $\delta_a$.
% as described in Appendix \ref{Appendix: downstream RL}. 
The target divergence $\delta_a$ is used to determine the parameter, $\alpha_a$, which determines the effect of the KL regularization term in the policy update objective as described in \cite{haarnoja2018soft, pertsch2021accelerating}. We compare $\delta_a$ values 10, 20, 50 and 80 for the maze navigation experiment corresponding to Fig. \ref{fig:MazeResults}. All methods are warm-started with SPiRL for 1M steps. Then they are trained via Skill-Critic with the varying value for $\delta_a$. The results show that when target divergence increases, the episode rewards increase correspondingly, because the LL policy has more freedom to deviate from the prior policy. Conversely, a smaller target divergence constrains the policy closer to the action prior, and Skill-Critic receives less reward. Furthermore, we provide the actual KL divergence of the LL policy from the action prior during training in the right of Fig. \ref{fig:Ablation_kl}. As explained on Line 9 in Algorithm \ref{Alg:low-level}, $\alpha_a$ is the dual gradient descent parameter to constrain the LL policy's divergence to the target divergence $\delta_a$. From the actual LL policy variance during training, we can see that the LL policy divergence is indeed constrained to the target divergence and converges to the target divergence value.

\textbf{LL Prior Distribution.} Skill-Prior RL \cite{pertsch2021accelerating} extends the uniform prior in SAC~\cite{haarnoja2018soft} to the non-uniform HL skill prior. Skill-Critic likewise employs a non-uniform action prior learned from demonstration to regularize the LL policy exploration. We conduct an ablation study in the maze navigation task using a uniform LL prior, which replaces the KL divergence regularization term with LL policy entropy. The results of the learning curves are provided in Fig. \ref{fig:Ablation}. We apply the auto entropy adjustment and use the target entropy value of -2~\cite{haarnoja2018soft2}. However, the uniform prior regularizes the LL policy to execute random actions, leading to inefficient exploration in the long-horizon environment.

\textbf{Variance of the Action Prior.} In Fig. \ref{fig:Ablation}, we change the variance of the action prior, $\sigma_{\hat{a}}$ to values $\log \sigma_{\hat{a}}=-1$, $-3$, and $-5$ in the maze navigation task. All methods are warm-started with SPiRL for 1M steps. Then they are trained via Skill-Critic with the varying value for $\sigma_{\hat{a}}$. When the variance is too small ($\log \sigma_{\hat{a}}=-5$), the LL policy is unable to sufficiently explore to improve its skills. Conversely, larger variance, i.e. $\log \sigma_{\hat{a}}=-1$, means the low-level policy explores with weaker regularization to the action prior, so the agent forgets previous skills and fails to reach the goal. We found a suitable value for the action-prior variance is $\log \sigma_{\hat{a}}=-3$, which promotes reasonable exploitation of the action prior and policy exploration to improve the skill set.

\end{newtext}



==> submit2/sections/intro_related.tex <==
% ============ intro =============
\section{Introduction} \label{Sec:Intro}

\IEEEPARstart{R}{einforcement} learning (RL) has demonstrated remarkable success in various domains~\cite{mnih2015human,  wurman2022outracing}. %zhang2023learning,
However, standard RL algorithms often lack the ability to incorporate prior structure, knowledge, or experience, which may be necessary for complex tasks~\cite{li2022hierarchical, pertsch2021accelerating, pertsch2021guided, singi2023decision}. Incorporating prior experience by learning from demonstrations can facilitate efficient exploration~\cite{argall2009survey}. For example, statistical methods can infer the hidden structure of offline data and inform the decision-making process~\cite{pertsch2021accelerating, pertsch2021guided}. However, offline data alone may not suffice for determining an optimal policy, particularly when the data originates from simpler environments or pertains to intricate or stochastic tasks. In such cases, online policy optimization (referred to as \textit{fine-tuning}) is required to refine suboptimal policies \cite{nair2020awac,  nakamoto2023cal}. We present a hierarchical RL framework that leverages offline data to accelerate RL training without limiting its performance by the quality of offline data. 



\begin{figure}
\centering
\includegraphics[width=0.3\textwidth, trim={0 2pt 0 3pt},clip]{figures/overview_new.pdf}
\caption{Skill-Critic leverages low-coverage demonstrations to facilitate hierarchical reinforcement learning by (1) acquiring a basic skill-set from demonstrations that (2) guides online skill selection and skill improvement.}
\end{figure}

Our framework employs \textit{skills}, temporally extended sequences of primitive actions~\cite{kingma2013auto}. Previous works extract skills from unstructured data and transfer them to downstream RL tasks with a skill selection policy whose action space is the skill itself~\cite{sharma2019dynamics}. Skill-Prior RL (SPiRL)~\cite{pertsch2021accelerating} found learning a set of skills may not be adequate to guide skill selection; rather, exploration is improved when high-level skill selection is regularized by a data-informed prior distribution known as the skill prior. The skill prior informs the high-level policy, but the low-level policy, i.e. the skill, is \emph{stationary}. However, with low-coverage or low-quality offline data, stationary skills may not suffice in complex downstream tasks. 

Our \emph{Skill-Critic} approach aims to leverage parallel high-level and low-level policy optimization to refine the skills themselves during skill selection. Intuitively, agents can use their experience to \textit{improve} their skill set, rather than being constrained to select skills from a stationary, offline library. 
We show this problem can be formulated as the parallel optimization of a high-level (HL) policy to select a skill and a low-level (LL) policy to select an action. We guide HL skill selection with a data-informed skill prior~\cite{pertsch2021accelerating}, and we extend this notion to initialize and regularize the LL skills using an action prior informed by offline data. Skill-Critic is reminiscent of discrete \textit{options}~\cite{zhang2019dac}; however, the offline data-informed, continuous skill space adds a unique structure for guiding and stabilizing the parallel policy optimization.


Our contributions are: (1) We formulate parallel optimization of the HL and LL policies to simultaneously select skills and improve the skill set, (2) We use an action prior to guide LL policy fine-tuning to improve the offline data-driven skill set, and (3) Our method \textit{improves} the skill set and performance in simulated navigation and robotic manipulation tasks and solves a new, sparse reward autonomous racing task in the complex Gran Turismo Sport environment.



% ========== related works =========
\section{Related Works} \label{Sec:RelatedWorks}

% \subsubsection{Offline RL}
% Offline RL algorithms use pre-collected demonstrations to learn optimal policies without environment interaction~\cite{levine2020offline}. When environment interaction is limited, offline RL can warm-start and accelerate online RL training~\cite{nair2020awac, singh2020cog, nakamoto2023cal}, which is referred to as \textit{fine-tuning}. However, the quality of offline priors highly relies on demonstrations. 
% RL fine-tuning performance can deteriorate when attempting to \textit{transfer} prior experience from one task to another~\cite{levine2020offline}. 

\subsubsection{Skill-transfer RL} 
Skill-transfer RL reuses pre-trained skills, i.e. sequences of actions, to accelerate RL training for downstream tasks~\cite{pertsch2021accelerating,pertsch2021guided, eysenbach2018diversity, hausman2018learning}. One commonly used approach is to learn a skill latent space from offline data using variational autoencoder (VAE)~\cite{kingma2013auto}. Then in downstream RL, an HL skill-selection policy is trained to select the optimal skill from the learned skill space. Thus, RL only needs to explore how to stitch temporally-extended action sequences, instead of searching for the optimal action at every time step. 
Extensions have learned priors for the HL policy from VAE training to guide and further accelerate RL training \cite{pertsch2021accelerating} and learned these skill priors from multiple datasets \cite{xu2022aspire}.
However, prior works often consider a \emph{stationary} skill space, constraining performance to skills learned from offline data. 
% Adaptive Skill-Prior RL (ASPiRe)~\cite{xu2022aspire} alleviates this issue by enabling the RL agent to compose skill priors learned from multiple datasets, but LL policies are still stationary. 
% Nevertheless, the LL policies are still stationary, and the RL agent may still fail when the downstream task requires skills unseen in any available datasets.
% It motivates us to propose Skill-Critic, which is a hierarchical RL method that can effectively leverage low-coverage 
% or low-quality data for skill-transfer RL. 

%chane2021goal

\subsubsection{Hierarchical RL} 
Hierarchical RL (HRL) decomposes long-horizon tasks into simpler sub-tasks, encouraging meaningful exploration during training~\cite{pateria2021hierarchical}. Commonly, algorithms employ intermediate variables, such as goals, options, or skills, to define subdomains that bridge high and low levels. Discrete options \cite{bacon2017option, zhang2019dac, li2020soac}  may not be sufficiently descriptive for complex tasks. Goal-conditioned HRL \cite{andrychowicz2017hindsight, eysenbach2022contrastive, nasiriany2019planning, pateria2021end, nachum2018data} leverages automatic goal sampling methods (e.g. from prior experience or demonstrations) to train goal-conditioned policies; however, goals must be available from the state space.
In Skill-transfer RL \cite{eysenbach2018diversity, hausman2018learning}, the hierarchical policies could use a data-informed, continuous latent space, potentially representing a wider range of behaviors. Recent works use residual policies to augment an LL data-driven skill decoder  \cite{rana2023residual, won2022physics}. Skill-Critic provides an alternate mechanism for parallel HL and LL policy optimization: the decoder is an \textit{action prior} to guide the LL policy, and the skill prior guides the HL policy.
% Parallel policy training can alleviate this issue, but may be unstable or more sample intensive than single-layer RL because the agent must explore both the intermediate space and action space~\cite{bacon2017option}.


% Goal-conditioning hierarchical RL \cite{gupta2019relay, li2022hierarchical} requires additional methods for automatically sampling goals, such as hindsight relabeling \cite{andrychowicz2017hindsight, levy2018learning} to label experiences using future outcomes. 

%Single-layer hierarchical RL (such as skill-transfer RL) may fail to adequately adjust to the downstream environment.
% Recent advances in goal-conditioned hierarchical learning 
% Parallel policy learning can be accelerated by pre-trained goal-conditioned 
% policies from demonstrations~\cite{gupta2019relay, li2022hierarchical, levy2018learning} that require structured goal states to be defined. Conversely, we leverage \textit{skills}, thereby adding structure and prior experience to guide the parallel policy optimization problem. 



